RIS-Enabled Self-Localization: Leveraging Controllable Reflections With Zero Access Points

Reconfigurable intelligent surfaces (RISs) are one of the most promising technological enablers of the next (6th) generation of wireless systems. In this paper, we introduce a novel use-case of the RIS technology in radio localization, which is enabling the user to estimate its own position via transmitting orthogonal frequency-division multiplexing (OFDM) pilots and processing the signal reflected from the RIS. We demonstrate that user localization in this scenario is possible by deriving Cramer-Rao lower bounds on the positioning error and devising a low-complexity position estimation algorithm. We consider random and directional RIS phase profiles and apply a specific temporal coding to them, such that the reflected signal from the RIS can be separated from the uncontrolled multipath. Finally, we assess the performance of our position estimator for an example system and show that the proposed algorithm can attain the derived bound at high signal-to-noise ratio values.

==> M.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
\definecolor{mycolor1}{rgb}{0.00000,0.44700,0.74100}%
\definecolor{mycolor2}{rgb}{0.85000,0.32500,0.09800}%
%

\begin{axis}[%
width=4.5cm,
height=4cm,
at={(9.5cm,0)},
scale only axis,
xmode=log,
xmin=100,
xmax=10000,
xminorticks=true,
ymode=log,
ymin=1e-04,
ymax=1,
xlabel={\footnotesize c) Number of RIS elements ($M$)},
ylabel={\footnotesize PEB [m]},
yminorticks=true,
axis background/.style={fill=white}
]
\node[rotate=-25,fill=white] at (axis cs:2000,.015) {\footnotesize Random };
\node[rotate=-35,fill=white] at (axis cs:2000,.001) {\footnotesize Directional };
%\draw (axis cs:5.5,.00004) ellipse (.1cm and .2cm);
%\draw (axis cs:5,.0005) ellipse (.1cm and .2cm);
\addplot [color=mycolor1, forget plot]
  table[row sep=crcr]{%
100	0.495942646021223\\
400	0.109543167415909\\
900	0.0492446649257843\\
1600	0.0309786253470164\\
2500	0.0195314078279764\\
3600	0.0124687046978132\\
4900	0.00935722782972363\\
6400	0.00767104517089799\\
8100	0.00577344553485302\\
10000	0.00471919321073767\\
12100	0.00395669664790676\\
14400	0.00332139309503642\\
16900	0.00263828068164294\\
19600	0.00209702561148599\\
22500	0.00201444501464538\\
};
\addplot [color=mycolor2, forget plot]
  table[row sep=crcr]{%
100	0.702776914361473\\
400	0.0451945364471025\\
900	0.00921489340438039\\
1600	0.00322692306481661\\
2500	0.00122364781191237\\
3600	0.000659564582258044\\
4900	0.00042445035332889\\
6400	0.000281239351516388\\
8100	0.000176241303779906\\
10000	0.000153799791019006\\
12100	0.000104150510755585\\
14400	9.53101678637555e-05\\
16900	7.28756874847079e-05\\
19600	8.21565367972888e-05\\
22500	6.00186975780037e-05\\
};
\end{axis}


==> RIS-Enabled Personal Radar/FigColorMaps.tex <==
\begin{tikzpicture}[every text node part/.style={align=center}]
\pgfplotsset{every tick label/.append style={font=\footnotesize}}
%%---------first image------------
\begin{axis}[
at={(8.95cm,0)},
axis on top,% ----
width=4.5cm,
height=4.5cm,
xlabel={\footnotesize $(a) \ \ x [\mathrm{m}]$},
scale only axis,
xmin=-20,
xmax=20,
ymin=0,
ymax=20,
%ytick=\empty,
enlargelimits=false, 
axis on top, 
]
\addplot[thick,blue] graphics[xmin=-20,ymin=0,xmax=20,ymax=20] {contour.pdf};
\end{axis}
\begin{axis}[at={(13.5cm,0cm)},axis on top,% ----
		width=.3cm,
		height=4.5cm,
		scale only axis,
		xmin=0,
		xmax=1,
		ymin=1e-4,
		ymax=1,
		ymode = log,
		xtick=\empty,
		%ytick style={ draw=none},
		%ytick={.02,.05,.1,.2,.4,.8},
        %yticklabels={$0.02$,$0.05$,$0.1$,$0.2$,$0.4$,$0.8$},
		enlargelimits=false, 
		axis on top, 
        ytick pos=right,
]
\addplot[thick,blue] graphics[xmin=0,ymin=1.04e-4,xmax=1,ymax=1] {ColorBar.png};
\end{axis}
\node [rotate = 90] at (8cm,2cm){\footnotesize $y[\mathrm{m}]$};
%--------------------------------------------
%%---------second image------------
\begin{axis}[
at={(8.95cm,-5.5cm)},
axis on top,% ----
width=4.5cm,
height=4.5cm,
xlabel={\footnotesize $(b) \ \ x [\mathrm{m}]$},
scale only axis,
xmin=-20,
xmax=20,
ymin=0,
ymax=20,
%ytick=\empty,
enlargelimits=false, 
axis on top, 
]
\addplot[thick,blue] graphics[xmin=-20,ymin=0,xmax=20,ymax=20] {contour2.pdf};
\end{axis}
\begin{axis}[at={(13.5cm,-5.5cm)},axis on top,% ----
		width=.3cm,
		height=4.5cm,
		scale only axis,
		xmin=0,
		xmax=1,
		ymin=7.47e-4,
		ymax=.02,
		ymode = log,
		xtick=\empty,
		%ytick style={ draw=none},
		%ytick={.02,.05,.1,.2,.4,.8},
        %yticklabels={$0.02$,$0.05$,$0.1$,$0.2$,$0.4$,$0.8$},
		enlargelimits=false, 
		axis on top, 
        ytick pos=right,
]
\addplot[thick,blue] graphics[xmin=0,ymin=7.47e-4,xmax=1,ymax=.02] {cb2.png};
\end{axis}
\node [rotate = 90] at (8cm,-4cm){\footnotesize $y[\mathrm{m}]$};
%--------------------------------------------
\end{tikzpicture}

==> RIS-Enabled Personal Radar/M.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
\definecolor{mycolor1}{rgb}{0.00000,0.44700,0.74100}%
\definecolor{mycolor2}{rgb}{0.85000,0.32500,0.09800}%
%

\begin{axis}[%
width=4.5cm,
height=4cm,
at={(9.5cm,0)},
scale only axis,
xmode=log,
xmin=100,
xmax=10000,
xminorticks=true,
ymode=log,
ymin=1e-04,
ymax=1,
xlabel={\footnotesize c) Number of RIS elements ($M$)},
ylabel={\footnotesize PEB [m]},
yminorticks=true,
axis background/.style={fill=white}
]
\node[rotate=-25,fill=white] at (axis cs:2000,.015) {\footnotesize Random };
\node[rotate=-35,fill=white] at (axis cs:2000,.001) {\footnotesize Directional };
%\draw (axis cs:5.5,.00004) ellipse (.1cm and .2cm);
%\draw (axis cs:5,.0005) ellipse (.1cm and .2cm);
\addplot [color=mycolor1, forget plot]
  table[row sep=crcr]{%
100	0.495942646021223\\
400	0.109543167415909\\
900	0.0492446649257843\\
1600	0.0309786253470164\\
2500	0.0195314078279764\\
3600	0.0124687046978132\\
4900	0.00935722782972363\\
6400	0.00767104517089799\\
8100	0.00577344553485302\\
10000	0.00471919321073767\\
12100	0.00395669664790676\\
14400	0.00332139309503642\\
16900	0.00263828068164294\\
19600	0.00209702561148599\\
22500	0.00201444501464538\\
};
\addplot [color=mycolor2, forget plot]
  table[row sep=crcr]{%
100	0.702776914361473\\
400	0.0451945364471025\\
900	0.00921489340438039\\
1600	0.00322692306481661\\
2500	0.00122364781191237\\
3600	0.000659564582258044\\
4900	0.00042445035332889\\
6400	0.000281239351516388\\
8100	0.000176241303779906\\
10000	0.000153799791019006\\
12100	0.000104150510755585\\
14400	9.53101678637555e-05\\
16900	7.28756874847079e-05\\
19600	8.21565367972888e-05\\
22500	6.00186975780037e-05\\
};
\end{axis}


==> RIS-Enabled Personal Radar/Results.tex <==
\definecolor{mycolor1}{rgb}{0.00000,0.44700,0.74100}%
\definecolor{mycolor2}{rgb}{0.85000,0.32500,0.09800}%
%
\begin{tikzpicture}[every text node part/.style={align=center}]
\pgfplotsset{every tick label/.append style={font=\footnotesize}}
\input{M}
\input{pebs}
\input{cdfs}
%--------------------
%\node [rotate = 0] at (0cm,4cm){\footnotesize (a)};
%\node [rotate = 0] at (6cm,4cm){\footnotesize (b)};
%\node [rotate = 0] at (11cm,4cm){\footnotesize (c)};
%\node [rotate = 90] at (8.3cm,2cm){\footnotesize $y[\mathrm{m}]$};
\node [rotate = 90] at (2.7cm,2cm){\footnotesize $\mathrm{Pr}(\mathrm{Error}<e)$};
\node [rotate = 90] at (-3.1cm,2cm){\footnotesize Positioning error $[\mathrm{m}]$};
\end{tikzpicture}


==> RIS-Enabled Personal Radar/cdfs.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
%\definecolor{mycolor1}{rgb}{0.00000,0.44700,0.74100}%
%\definecolor{mycolor2}{rgb}{0.85000,0.32500,0.09800}%
%

\begin{axis}[%
at={(3.5cm,0)},
width=4.5cm,
height=4cm,
scale only axis,
unbounded coords=jump,
xmode=log,
xmin=1e-4,
xmax=0.03,
xminorticks=true,
xlabel style={font=\color{white!15!black}},
xlabel={\footnotesize $b) e[\mathrm{m}]$},
ymin=0,
ymax=1,
axis background/.style={fill=white},
title style={font=\bfseries},
axis x line*=bottom,
axis y line*=left,
xmajorgrids,
xminorgrids,
ymajorgrids
]
\node[rotate=0,fill=white] at (axis cs:.003,.6) {\footnotesize Random};
\node[rotate=0,fill=white] at (axis cs:.0006,.5) {\footnotesize Directional};
\draw (axis cs:.007,.6) ellipse (.2cm and .1cm);
\draw (axis cs:.0002,.5) ellipse (.2cm and .1cm);
\addplot [color=mycolor2, forget plot,line width=1.5,dashed]
  table[row sep=crcr]{%
-inf	0\\
0.00388763495332524	0\\
0.00388763495332524	0.01\\
0.0039779769369078	0.01\\
0.0039779769369078	0.02\\
0.00437702219895772	0.02\\
0.00437702219895772	0.03\\
0.0045279377194668	0.03\\
0.0045279377194668	0.04\\
0.00456982329175554	0.04\\
0.00456982329175554	0.05\\
0.00483098405479953	0.05\\
0.00483098405479953	0.06\\
0.00494256970577131	0.06\\
0.00494256970577131	0.07\\
0.00501030301268805	0.07\\
0.00501030301268805	0.08\\
0.00513783394341532	0.08\\
0.00513783394341532	0.09\\
0.00519586445469606	0.09\\
0.00519586445469606	0.1\\
0.00523357784167244	0.1\\
0.00523357784167244	0.11\\
0.00525944393745265	0.11\\
0.00525944393745265	0.12\\
0.00531603796773738	0.12\\
0.00531603796773738	0.13\\
0.00541826257025269	0.13\\
0.00541826257025269	0.14\\
0.00543579830221148	0.14\\
0.00543579830221148	0.15\\
0.00547540416269369	0.15\\
0.00547540416269369	0.16\\
0.0054851530725855	0.16\\
0.0054851530725855	0.17\\
0.00550140659815427	0.17\\
0.00550140659815427	0.18\\
0.00552060998763975	0.18\\
0.00552060998763975	0.19\\
0.00555979050277402	0.19\\
0.00555979050277402	0.2\\
0.00556285059006915	0.2\\
0.00556285059006915	0.21\\
0.00568453435581969	0.21\\
0.00568453435581969	0.22\\
0.00569204200507351	0.22\\
0.00569204200507351	0.23\\
0.00579280694758293	0.23\\
0.00579280694758293	0.24\\
0.00579995431037703	0.24\\
0.00579995431037703	0.25\\
0.00588773873775303	0.25\\
0.00588773873775303	0.26\\
0.00593842205392088	0.26\\
0.00593842205392088	0.27\\
0.00603254823975779	0.27\\
0.00603254823975779	0.28\\
0.00612865636514691	0.28\\
0.00612865636514691	0.29\\
0.0061630099478404	0.29\\
0.0061630099478404	0.3\\
0.00617432934146672	0.3\\
0.00617432934146672	0.31\\
0.00618994226040939	0.31\\
0.00618994226040939	0.32\\
0.00620976839154533	0.32\\
0.00620976839154533	0.33\\
0.00621589041047224	0.33\\
0.00621589041047224	0.34\\
0.00622299644651732	0.34\\
0.00622299644651732	0.35\\
0.0062343259165862	0.35\\
0.0062343259165862	0.36\\
0.00627648039045602	0.36\\
0.00627648039045602	0.37\\
0.00634545501416627	0.37\\
0.00634545501416627	0.38\\
0.00637730768160198	0.38\\
0.00637730768160198	0.39\\
0.00640788564009761	0.39\\
0.00640788564009761	0.4\\
0.006415855404117	0.4\\
0.006415855404117	0.41\\
0.00646372169868585	0.41\\
0.00646372169868585	0.42\\
0.00654699862180399	0.42\\
0.00654699862180399	0.43\\
0.00656728063394036	0.43\\
0.00656728063394036	0.44\\
0.00658800268562385	0.44\\
0.00658800268562385	0.45\\
0.00661947482080476	0.45\\
0.00661947482080476	0.46\\
0.00671287872309909	0.46\\
0.00671287872309909	0.47\\
0.00673209634434497	0.47\\
0.00673209634434497	0.48\\
0.00673873996814358	0.48\\
0.00673873996814358	0.49\\
0.00676493352657311	0.49\\
0.00676493352657311	0.5\\
0.00678293182547686	0.5\\
0.00678293182547686	0.51\\
0.0067864636826908	0.51\\
0.0067864636826908	0.52\\
0.00688843352181448	0.52\\
0.00688843352181448	0.53\\
0.00690218623404389	0.53\\
0.00690218623404389	0.54\\
0.00692059412019435	0.54\\
0.00692059412019435	0.55\\
0.00695228513937172	0.55\\
0.00695228513937172	0.56\\
0.00696268765805748	0.56\\
0.00696268765805748	0.57\\
0.00698901995086007	0.57\\
0.00698901995086007	0.58\\
0.00701887482569471	0.58\\
0.00701887482569471	0.59\\
0.0070881888437203	0.59\\
0.0070881888437203	0.6\\
0.00709133457158546	0.6\\
0.00709133457158546	0.61\\
0.00709938665983232	0.61\\
0.00709938665983232	0.62\\
0.0071103192620758	0.62\\
0.0071103192620758	0.63\\
0.00714802314516168	0.63\\
0.00714802314516168	0.64\\
0.00717948379555864	0.64\\
0.00717948379555864	0.65\\
0.00720661799340744	0.65\\
0.00720661799340744	0.66\\
0.00721072490628053	0.66\\
0.00721072490628053	0.67\\
0.00727713275796887	0.67\\
0.00727713275796887	0.68\\
0.00733014380839564	0.68\\
0.00733014380839564	0.69\\
0.00734040335966124	0.69\\
0.00734040335966124	0.7\\
0.00736378800319066	0.7\\
0.00736378800319066	0.71\\
0.00736572374519651	0.71\\
0.00736572374519651	0.72\\
0.0073765123257748	0.72\\
0.0073765123257748	0.73\\
0.00741673477843082	0.73\\
0.00741673477843082	0.74\\
0.00749952340862622	0.74\\
0.00749952340862622	0.75\\
0.00753265357893415	0.75\\
0.00753265357893415	0.76\\
0.00754037977442961	0.76\\
0.00754037977442961	0.77\\
0.00758943452362781	0.77\\
0.00758943452362781	0.78\\
0.00761475721000997	0.78\\
0.00761475721000997	0.79\\
0.0077412746042716	0.79\\
0.0077412746042716	0.8\\
0.00776843123485257	0.8\\
0.00776843123485257	0.81\\
0.00783275913583604	0.81\\
0.00783275913583604	0.82\\
0.00791905001768998	0.82\\
0.00791905001768998	0.83\\
0.00807806751081398	0.83\\
0.00807806751081398	0.84\\
0.00813986797387923	0.84\\
0.00813986797387923	0.85\\
0.00825723615635137	0.85\\
0.00825723615635137	0.86\\
0.0082713869507189	0.86\\
0.0082713869507189	0.87\\
0.00831161454742953	0.87\\
0.00831161454742953	0.88\\
0.00851917175990109	0.88\\
0.00851917175990109	0.89\\
0.0085322476072092	0.89\\
0.0085322476072092	0.9\\
0.00861277743903294	0.9\\
0.00861277743903294	0.91\\
0.00865109615772425	0.91\\
0.00865109615772425	0.92\\
0.00872005431699495	0.92\\
0.00872005431699495	0.93\\
0.00872265152206257	0.93\\
0.00872265152206257	0.94\\
0.00880711469000858	0.94\\
0.00880711469000858	0.95\\
0.00888147476122421	0.95\\
0.00888147476122421	0.96\\
0.00943840673278368	0.96\\
0.00943840673278368	0.97\\
0.00945555000782478	0.97\\
0.00945555000782478	0.98\\
0.00978202883359448	0.98\\
0.00978202883359448	0.99\\
0.00994107140898879	0.99\\
0.00994107140898879	1\\
inf	1\\
};
\node[rotate=0,fill=white] at (axis cs:.0006,.5) {\footnotesize Directional};
\draw (axis cs:.007,.6) ellipse (.2cm and .1cm);
\draw (axis cs:.0002,.5) ellipse (.2cm and .1cm);
\addplot [color=mycolor2, forget plot,line width=1.5,dashed]
  table[row sep=crcr]{%
-inf	0\\
0.00388763495332524	0\\
0.00388763495332524	0.01\\
0.0039779769369078	0.01\\
0.0039779769369078	0.02\\
0.00437702219895772	0.02\\
0.00437702219895772	0.03\\
0.0045279377194668	0.03\\
0.0045279377194668	0.04\\
0.00456982329175554	0.04\\
0.00456982329175554	0.05\\
0.00483098405479953	0.05\\
0.00483098405479953	0.06\\
0.00494256970577131	0.06\\
0.00494256970577131	0.07\\
0.00501030301268805	0.07\\
0.00501030301268805	0.08\\
0.00513783394341532	0.08\\
0.00513783394341532	0.09\\
0.00519586445469606	0.09\\
0.00519586445469606	0.1\\
0.00523357784167244	0.1\\
0.00523357784167244	0.11\\
0.00525944393745265	0.11\\
0.00525944393745265	0.12\\
0.00531603796773738	0.12\\
0.00531603796773738	0.13\\
0.00541826257025269	0.13\\
0.00541826257025269	0.14\\
0.00543579830221148	0.14\\
0.00543579830221148	0.15\\
0.00547540416269369	0.15\\
0.00547540416269369	0.16\\
0.0054851530725855	0.16\\
0.0054851530725855	0.17\\
0.00550140659815427	0.17\\
0.00550140659815427	0.18\\
0.00552060998763975	0.18\\
0.00552060998763975	0.19\\
0.00555979050277402	0.19\\
0.00555979050277402	0.2\\
0.00556285059006915	0.2\\
0.00556285059006915	0.21\\
0.00568453435581969	0.21\\
0.00568453435581969	0.22\\
0.00569204200507351	0.22\\
0.00569204200507351	0.23\\
0.00579280694758293	0.23\\
0.00579280694758293	0.24\\
0.00579995431037703	0.24\\
0.00579995431037703	0.25\\
0.00588773873775303	0.25\\
0.00588773873775303	0.26\\
0.00593842205392088	0.26\\
0.00593842205392088	0.27\\
0.00603254823975779	0.27\\
0.00603254823975779	0.28\\
0.00612865636514691	0.28\\
0.00612865636514691	0.29\\
0.0061630099478404	0.29\\
0.0061630099478404	0.3\\
0.00617432934146672	0.3\\
0.00617432934146672	0.31\\
0.00618994226040939	0.31\\
0.00618994226040939	0.32\\
0.00620976839154533	0.32\\
0.00620976839154533	0.33\\
0.00621589041047224	0.33\\
0.00621589041047224	0.34\\
0.00622299644651732	0.34\\
0.00622299644651732	0.35\\
0.0062343259165862	0.35\\
0.0062343259165862	0.36\\
0.00627648039045602	0.36\\
0.00627648039045602	0.37\\
0.00634545501416627	0.37\\
0.00634545501416627	0.38\\
0.00637730768160198	0.38\\
0.00637730768160198	0.39\\
0.00640788564009761	0.39\\
0.00640788564009761	0.4\\
0.006415855404117	0.4\\
0.006415855404117	0.41\\
0.00646372169868585	0.41\\
0.00646372169868585	0.42\\
0.00654699862180399	0.42\\
0.00654699862180399	0.43\\
0.00656728063394036	0.43\\
0.00656728063394036	0.44\\
0.00658800268562385	0.44\\
0.00658800268562385	0.45\\
0.00661947482080476	0.45\\
0.00661947482080476	0.46\\
0.00671287872309909	0.46\\
0.00671287872309909	0.47\\
0.00673209634434497	0.47\\
0.00673209634434497	0.48\\
0.00673873996814358	0.48\\
0.00673873996814358	0.49\\
0.00676493352657311	0.49\\
0.00676493352657311	0.5\\
0.00678293182547686	0.5\\
0.00678293182547686	0.51\\
0.0067864636826908	0.51\\
0.0067864636826908	0.52\\
0.00688843352181448	0.52\\
0.00688843352181448	0.53\\
0.00690218623404389	0.53\\
0.00690218623404389	0.54\\
0.00692059412019435	0.54\\
0.00692059412019435	0.55\\
0.00695228513937172	0.55\\
0.00695228513937172	0.56\\
0.00696268765805748	0.56\\
0.00696268765805748	0.57\\
0.00698901995086007	0.57\\
0.00698901995086007	0.58\\
0.00701887482569471	0.58\\
0.00701887482569471	0.59\\
0.0070881888437203	0.59\\
0.0070881888437203	0.6\\
0.00709133457158546	0.6\\
0.00709133457158546	0.61\\
0.00709938665983232	0.61\\
0.00709938665983232	0.62\\
0.0071103192620758	0.62\\
0.0071103192620758	0.63\\
0.00714802314516168	0.63\\
0.00714802314516168	0.64\\
0.00717948379555864	0.64\\
0.00717948379555864	0.65\\
0.00720661799340744	0.65\\
0.00720661799340744	0.66\\
0.00721072490628053	0.66\\
0.00721072490628053	0.67\\
0.00727713275796887	0.67\\
0.00727713275796887	0.68\\
0.00733014380839564	0.68\\
0.00733014380839564	0.69\\
0.00734040335966124	0.69\\
0.00734040335966124	0.7\\
0.00736378800319066	0.7\\
0.00736378800319066	0.71\\
0.00736572374519651	0.71\\
0.00736572374519651	0.72\\
0.0073765123257748	0.72\\
0.0073765123257748	0.73\\
0.00741673477843082	0.73\\
0.00741673477843082	0.74\\
0.00749952340862622	0.74\\
0.00749952340862622	0.75\\
0.00753265357893415	0.75\\
0.00753265357893415	0.76\\
0.00754037977442961	0.76\\
0.00754037977442961	0.77\\
0.00758943452362781	0.77\\
0.00758943452362781	0.78\\
0.00761475721000997	0.78\\
0.00761475721000997	0.79\\
0.0077412746042716	0.79\\
0.0077412746042716	0.8\\
0.00776843123485257	0.8\\
0.00776843123485257	0.81\\
0.00783275913583604	0.81\\
0.00783275913583604	0.82\\
0.00791905001768998	0.82\\
0.00791905001768998	0.83\\
0.00807806751081398	0.83\\
0.00807806751081398	0.84\\
0.00813986797387923	0.84\\
0.00813986797387923	0.85\\
0.00825723615635137	0.85\\
0.00825723615635137	0.86\\
0.0082713869507189	0.86\\
0.0082713869507189	0.87\\
0.00831161454742953	0.87\\
0.00831161454742953	0.88\\
0.00851917175990109	0.88\\
0.00851917175990109	0.89\\
0.0085322476072092	0.89\\
0.0085322476072092	0.9\\
0.00861277743903294	0.9\\
0.00861277743903294	0.91\\
0.00865109615772425	0.91\\
0.00865109615772425	0.92\\
0.00872005431699495	0.92\\
0.00872005431699495	0.93\\
0.00872265152206257	0.93\\
0.00872265152206257	0.94\\
0.00880711469000858	0.94\\
0.00880711469000858	0.95\\
0.00888147476122421	0.95\\
0.00888147476122421	0.96\\
0.00943840673278368	0.96\\
0.00943840673278368	0.97\\
0.00945555000782478	0.97\\
0.00945555000782478	0.98\\
0.00978202883359448	0.98\\
0.00978202883359448	0.99\\
0.00994107140898879	0.99\\
0.00994107140898879	1\\
inf	1\\
};
\addplot [color=mycolor1, forget plot,line width=1.5]
  table[row sep=crcr]{%
-inf	0\\
0.00594100985237028	0\\
0.00594100985237028	0.01\\
0.00599009318527625	0.01\\
0.00599009318527625	0.02\\
0.00608293910923256	0.02\\
0.00608293910923256	0.03\\
0.00612100166685542	0.03\\
0.00612100166685542	0.04\\
0.0061438320642927	0.04\\
0.0061438320642927	0.05\\
0.00619205557790499	0.05\\
0.00619205557790499	0.06\\
0.00620959461818174	0.06\\
0.00620959461818174	0.07\\
0.00626229810250843	0.07\\
0.00626229810250843	0.08\\
0.00628484051723775	0.08\\
0.00628484051723775	0.09\\
0.00628787260249079	0.09\\
0.00628787260249079	0.1\\
0.00630051532259005	0.1\\
0.00630051532259005	0.11\\
0.00630513895786879	0.11\\
0.00630513895786879	0.12\\
0.00639814449263139	0.12\\
0.00639814449263139	0.13\\
0.00639999018185661	0.13\\
0.00639999018185661	0.14\\
0.00642100695036684	0.14\\
0.00642100695036684	0.15\\
0.0064223267240867	0.15\\
0.0064223267240867	0.16\\
0.00644484772732915	0.16\\
0.00644484772732915	0.17\\
0.00648379520670121	0.17\\
0.00648379520670121	0.18\\
0.00648595849995988	0.18\\
0.00648595849995988	0.19\\
0.0065160669128008	0.19\\
0.0065160669128008	0.2\\
0.00651800783203751	0.2\\
0.00651800783203751	0.21\\
0.00653780348947287	0.21\\
0.00653780348947287	0.22\\
0.00655071835161352	0.22\\
0.00655071835161352	0.23\\
0.00655097699606874	0.23\\
0.00655097699606874	0.24\\
0.00656035999919366	0.24\\
0.00656035999919366	0.25\\
0.00656521033430283	0.25\\
0.00656521033430283	0.26\\
0.00656770409220368	0.26\\
0.00656770409220368	0.27\\
0.00657314285487407	0.27\\
0.00657314285487407	0.28\\
0.00660724824334752	0.28\\
0.00660724824334752	0.29\\
0.00661443603215063	0.29\\
0.00661443603215063	0.3\\
0.00661949165534638	0.3\\
0.00661949165534638	0.31\\
0.00662172939798818	0.31\\
0.00662172939798818	0.32\\
0.0066234818202168	0.32\\
0.0066234818202168	0.33\\
0.00663655304330502	0.33\\
0.00663655304330502	0.34\\
0.00666537258185465	0.34\\
0.00666537258185465	0.35\\
0.00666997356377142	0.35\\
0.00666997356377142	0.36\\
0.00668990634013947	0.36\\
0.00668990634013947	0.37\\
0.00669850296160555	0.37\\
0.00669850296160555	0.38\\
0.00672666207867346	0.38\\
0.00672666207867346	0.39\\
0.00672793821785664	0.39\\
0.00672793821785664	0.4\\
0.00673900999319645	0.4\\
0.00673900999319645	0.41\\
0.0067480603076519	0.41\\
0.0067480603076519	0.42\\
0.00679255448276614	0.42\\
0.00679255448276614	0.43\\
0.00680142826592546	0.43\\
0.00680142826592546	0.44\\
0.00680652403559258	0.44\\
0.00680652403559258	0.45\\
0.0068112915584925	0.45\\
0.0068112915584925	0.46\\
0.0068114050883781	0.46\\
0.0068114050883781	0.47\\
0.00681325895554897	0.47\\
0.00681325895554897	0.48\\
0.00682774836370451	0.48\\
0.00682774836370451	0.49\\
0.00682867776816079	0.49\\
0.00682867776816079	0.5\\
0.00686081372727172	0.5\\
0.00686081372727172	0.51\\
0.00687319130309085	0.51\\
0.00687319130309085	0.52\\
0.00687560549718734	0.52\\
0.00687560549718734	0.53\\
0.00688041209843295	0.53\\
0.00688041209843295	0.54\\
0.00688322308744301	0.54\\
0.00688322308744301	0.55\\
0.00689341480763436	0.55\\
0.00689341480763436	0.56\\
0.00690180459866101	0.56\\
0.00690180459866101	0.57\\
0.00690631648921724	0.57\\
0.00690631648921724	0.58\\
0.00692350250255314	0.58\\
0.00692350250255314	0.59\\
0.00692415714623772	0.59\\
0.00692415714623772	0.6\\
0.00692706459492213	0.6\\
0.00692706459492213	0.61\\
0.00692811521293472	0.61\\
0.00692811521293472	0.62\\
0.00694132508060988	0.62\\
0.00694132508060988	0.63\\
0.00694747027538867	0.63\\
0.00694747027538867	0.64\\
0.00696447902670257	0.64\\
0.00696447902670257	0.65\\
0.00697885218236809	0.65\\
0.00697885218236809	0.66\\
0.00697998994538625	0.66\\
0.00697998994538625	0.67\\
0.00698089026183617	0.67\\
0.00698089026183617	0.68\\
0.00698886050575452	0.68\\
0.00698886050575452	0.69\\
0.00699347728704452	0.69\\
0.00699347728704452	0.7\\
0.00699445228160716	0.7\\
0.00699445228160716	0.71\\
0.00700024363357147	0.71\\
0.00700024363357147	0.72\\
0.00703515647796582	0.72\\
0.00703515647796582	0.73\\
0.00705293919011259	0.73\\
0.00705293919011259	0.74\\
0.00706666840442122	0.74\\
0.00706666840442122	0.75\\
0.00707374338173634	0.75\\
0.00707374338173634	0.76\\
0.00707935883172926	0.76\\
0.00707935883172926	0.77\\
0.00708973165635371	0.77\\
0.00708973165635371	0.78\\
0.00709033204312792	0.78\\
0.00709033204312792	0.79\\
0.00712502611020385	0.79\\
0.00712502611020385	0.8\\
0.00714302264006296	0.8\\
0.00714302264006296	0.81\\
0.00715106481882321	0.81\\
0.00715106481882321	0.82\\
0.00715558175162197	0.82\\
0.00715558175162197	0.83\\
0.00716296788994827	0.83\\
0.00716296788994827	0.84\\
0.0071717992877789	0.84\\
0.0071717992877789	0.85\\
0.00719582884520419	0.85\\
0.00719582884520419	0.86\\
0.00719978994612414	0.86\\
0.00719978994612414	0.87\\
0.00725214656916683	0.87\\
0.00725214656916683	0.88\\
0.0072559042471206	0.88\\
0.0072559042471206	0.89\\
0.00727206028014622	0.89\\
0.00727206028014622	0.9\\
0.0073002894567794	0.9\\
0.0073002894567794	0.91\\
0.00730865983457664	0.91\\
0.00730865983457664	0.92\\
0.00732552008791973	0.92\\
0.00732552008791973	0.93\\
0.00740587093370403	0.93\\
0.00740587093370403	0.94\\
0.00743721550781977	0.94\\
0.00743721550781977	0.95\\
0.00754312957575401	0.95\\
0.00754312957575401	0.96\\
0.00760432749786826	0.96\\
0.00760432749786826	0.97\\
0.00766434998081241	0.97\\
0.00766434998081241	0.98\\
0.00768174563188015	0.98\\
0.00768174563188015	0.99\\
0.00778197997001614	0.99\\
0.00778197997001614	1\\
inf	1\\
};
\draw (axis cs:.007,.6) ellipse (.2cm and .1cm);
\draw (axis cs:.0002,.5) ellipse (.2cm and .1cm);
\addplot [color=mycolor2, forget plot,line width=1.5,dashed]
  table[row sep=crcr]{%
-inf	0\\
0.00388763495332524	0\\
0.00388763495332524	0.01\\
0.0039779769369078	0.01\\
0.0039779769369078	0.02\\
0.00437702219895772	0.02\\
0.00437702219895772	0.03\\
0.0045279377194668	0.03\\
0.0045279377194668	0.04\\
0.00456982329175554	0.04\\
0.00456982329175554	0.05\\
0.00483098405479953	0.05\\
0.00483098405479953	0.06\\
0.00494256970577131	0.06\\
0.00494256970577131	0.07\\
0.00501030301268805	0.07\\
0.00501030301268805	0.08\\
0.00513783394341532	0.08\\
0.00513783394341532	0.09\\
0.00519586445469606	0.09\\
0.00519586445469606	0.1\\
0.00523357784167244	0.1\\
0.00523357784167244	0.11\\
0.00525944393745265	0.11\\
0.00525944393745265	0.12\\
0.00531603796773738	0.12\\
0.00531603796773738	0.13\\
0.00541826257025269	0.13\\
0.00541826257025269	0.14\\
0.00543579830221148	0.14\\
0.00543579830221148	0.15\\
0.00547540416269369	0.15\\
0.00547540416269369	0.16\\
0.0054851530725855	0.16\\
0.0054851530725855	0.17\\
0.00550140659815427	0.17\\
0.00550140659815427	0.18\\
0.00552060998763975	0.18\\
0.00552060998763975	0.19\\
0.00555979050277402	0.19\\
0.00555979050277402	0.2\\
0.00556285059006915	0.2\\
0.00556285059006915	0.21\\
0.00568453435581969	0.21\\
0.00568453435581969	0.22\\
0.00569204200507351	0.22\\
0.00569204200507351	0.23\\
0.00579280694758293	0.23\\
0.00579280694758293	0.24\\
0.00579995431037703	0.24\\
0.00579995431037703	0.25\\
0.00588773873775303	0.25\\
0.00588773873775303	0.26\\
0.00593842205392088	0.26\\
0.00593842205392088	0.27\\
0.00603254823975779	0.27\\
0.00603254823975779	0.28\\
0.00612865636514691	0.28\\
0.00612865636514691	0.29\\
0.0061630099478404	0.29\\
0.0061630099478404	0.3\\
0.00617432934146672	0.3\\
0.00617432934146672	0.31\\
0.00618994226040939	0.31\\
0.00618994226040939	0.32\\
0.00620976839154533	0.32\\
0.00620976839154533	0.33\\
0.00621589041047224	0.33\\
0.00621589041047224	0.34\\
0.00622299644651732	0.34\\
0.00622299644651732	0.35\\
0.0062343259165862	0.35\\
0.0062343259165862	0.36\\
0.00627648039045602	0.36\\
0.00627648039045602	0.37\\
0.00634545501416627	0.37\\
0.00634545501416627	0.38\\
0.00637730768160198	0.38\\
0.00637730768160198	0.39\\
0.00640788564009761	0.39\\
0.00640788564009761	0.4\\
0.006415855404117	0.4\\
0.006415855404117	0.41\\
0.00646372169868585	0.41\\
0.00646372169868585	0.42\\
0.00654699862180399	0.42\\
0.00654699862180399	0.43\\
0.00656728063394036	0.43\\
0.00656728063394036	0.44\\
0.00658800268562385	0.44\\
0.00658800268562385	0.45\\
0.00661947482080476	0.45\\
0.00661947482080476	0.46\\
0.00671287872309909	0.46\\
0.00671287872309909	0.47\\
0.00673209634434497	0.47\\
0.00673209634434497	0.48\\
0.00673873996814358	0.48\\
0.00673873996814358	0.49\\
0.00676493352657311	0.49\\
0.00676493352657311	0.5\\
0.00678293182547686	0.5\\
0.00678293182547686	0.51\\
0.0067864636826908	0.51\\
0.0067864636826908	0.52\\
0.00688843352181448	0.52\\
0.00688843352181448	0.53\\
0.00690218623404389	0.53\\
0.00690218623404389	0.54\\
0.00692059412019435	0.54\\
0.00692059412019435	0.55\\
0.00695228513937172	0.55\\
0.00695228513937172	0.56\\
0.00696268765805748	0.56\\
0.00696268765805748	0.57\\
0.00698901995086007	0.57\\
0.00698901995086007	0.58\\
0.00701887482569471	0.58\\
0.00701887482569471	0.59\\
0.0070881888437203	0.59\\
0.0070881888437203	0.6\\
0.00709133457158546	0.6\\
0.00709133457158546	0.61\\
0.00709938665983232	0.61\\
0.00709938665983232	0.62\\
0.0071103192620758	0.62\\
0.0071103192620758	0.63\\
0.00714802314516168	0.63\\
0.00714802314516168	0.64\\
0.00717948379555864	0.64\\
0.00717948379555864	0.65\\
0.00720661799340744	0.65\\
0.00720661799340744	0.66\\
0.00721072490628053	0.66\\
0.00721072490628053	0.67\\
0.00727713275796887	0.67\\
0.00727713275796887	0.68\\
0.00733014380839564	0.68\\
0.00733014380839564	0.69\\
0.00734040335966124	0.69\\
0.00734040335966124	0.7\\
0.00736378800319066	0.7\\
0.00736378800319066	0.71\\
0.00736572374519651	0.71\\
0.00736572374519651	0.72\\
0.0073765123257748	0.72\\
0.0073765123257748	0.73\\
0.00741673477843082	0.73\\
0.00741673477843082	0.74\\
0.00749952340862622	0.74\\
0.00749952340862622	0.75\\
0.00753265357893415	0.75\\
0.00753265357893415	0.76\\
0.00754037977442961	0.76\\
0.00754037977442961	0.77\\
0.00758943452362781	0.77\\
0.00758943452362781	0.78\\
0.00761475721000997	0.78\\
0.00761475721000997	0.79\\
0.0077412746042716	0.79\\
0.0077412746042716	0.8\\
0.00776843123485257	0.8\\
0.00776843123485257	0.81\\
0.00783275913583604	0.81\\
0.00783275913583604	0.82\\
0.00791905001768998	0.82\\
0.00791905001768998	0.83\\
0.00807806751081398	0.83\\
0.00807806751081398	0.84\\
0.00813986797387923	0.84\\
0.00813986797387923	0.85\\
0.00825723615635137	0.85\\
0.00825723615635137	0.86\\
0.0082713869507189	0.86\\
0.0082713869507189	0.87\\
0.00831161454742953	0.87\\
0.00831161454742953	0.88\\
0.00851917175990109	0.88\\
0.00851917175990109	0.89\\
0.0085322476072092	0.89\\
0.0085322476072092	0.9\\
0.00861277743903294	0.9\\
0.00861277743903294	0.91\\
0.00865109615772425	0.91\\
0.00865109615772425	0.92\\
0.00872005431699495	0.92\\
0.00872005431699495	0.93\\
0.00872265152206257	0.93\\
0.00872265152206257	0.94\\
0.00880711469000858	0.94\\
0.00880711469000858	0.95\\
0.00888147476122421	0.95\\
0.00888147476122421	0.96\\
0.00943840673278368	0.96\\
0.00943840673278368	0.97\\
0.00945555000782478	0.97\\
0.00945555000782478	0.98\\
0.00978202883359448	0.98\\
0.00978202883359448	0.99\\
0.00994107140898879	0.99\\
0.00994107140898879	1\\
inf	1\\
};
\addplot [color=mycolor1, forget plot,line width=1.5]
  table[row sep=crcr]{%
-inf	0\\
0.00594100985237028	0\\
0.00594100985237028	0.01\\
0.00599009318527625	0.01\\
0.00599009318527625	0.02\\
0.00608293910923256	0.02\\
0.00608293910923256	0.03\\
0.00612100166685542	0.03\\
0.00612100166685542	0.04\\
0.0061438320642927	0.04\\
0.0061438320642927	0.05\\
0.00619205557790499	0.05\\
0.00619205557790499	0.06\\
0.00620959461818174	0.06\\
0.00620959461818174	0.07\\
0.00626229810250843	0.07\\
0.00626229810250843	0.08\\
0.00628484051723775	0.08\\
0.00628484051723775	0.09\\
0.00628787260249079	0.09\\
0.00628787260249079	0.1\\
0.00630051532259005	0.1\\
0.00630051532259005	0.11\\
0.00630513895786879	0.11\\
0.00630513895786879	0.12\\
0.00639814449263139	0.12\\
0.00639814449263139	0.13\\
0.00639999018185661	0.13\\
0.00639999018185661	0.14\\
0.00642100695036684	0.14\\
0.00642100695036684	0.15\\
0.0064223267240867	0.15\\
0.0064223267240867	0.16\\
0.00644484772732915	0.16\\
0.00644484772732915	0.17\\
0.00648379520670121	0.17\\
0.00648379520670121	0.18\\
0.00648595849995988	0.18\\
0.00648595849995988	0.19\\
0.0065160669128008	0.19\\
0.0065160669128008	0.2\\
0.00651800783203751	0.2\\
0.00651800783203751	0.21\\
0.00653780348947287	0.21\\
0.00653780348947287	0.22\\
0.00655071835161352	0.22\\
0.00655071835161352	0.23\\
0.00655097699606874	0.23\\
0.00655097699606874	0.24\\
0.00656035999919366	0.24\\
0.00656035999919366	0.25\\
0.00656521033430283	0.25\\
0.00656521033430283	0.26\\
0.00656770409220368	0.26\\
0.00656770409220368	0.27\\
0.00657314285487407	0.27\\
0.00657314285487407	0.28\\
0.00660724824334752	0.28\\
0.00660724824334752	0.29\\
0.00661443603215063	0.29\\
0.00661443603215063	0.3\\
0.00661949165534638	0.3\\
0.00661949165534638	0.31\\
0.00662172939798818	0.31\\
0.00662172939798818	0.32\\
0.0066234818202168	0.32\\
0.0066234818202168	0.33\\
0.00663655304330502	0.33\\
0.00663655304330502	0.34\\
0.00666537258185465	0.34\\
0.00666537258185465	0.35\\
0.00666997356377142	0.35\\
0.00666997356377142	0.36\\
0.00668990634013947	0.36\\
0.00668990634013947	0.37\\
0.00669850296160555	0.37\\
0.00669850296160555	0.38\\
0.00672666207867346	0.38\\
0.00672666207867346	0.39\\
0.00672793821785664	0.39\\
0.00672793821785664	0.4\\
0.00673900999319645	0.4\\
0.00673900999319645	0.41\\
0.0067480603076519	0.41\\
0.0067480603076519	0.42\\
0.00679255448276614	0.42\\
0.00679255448276614	0.43\\
0.00680142826592546	0.43\\
0.00680142826592546	0.44\\
0.00680652403559258	0.44\\
0.00680652403559258	0.45\\
0.0068112915584925	0.45\\
0.0068112915584925	0.46\\
0.0068114050883781	0.46\\
0.0068114050883781	0.47\\
0.00681325895554897	0.47\\
0.00681325895554897	0.48\\
0.00682774836370451	0.48\\
0.00682774836370451	0.49\\
0.00682867776816079	0.49\\
0.00682867776816079	0.5\\
0.00686081372727172	0.5\\
0.00686081372727172	0.51\\
0.00687319130309085	0.51\\
0.00687319130309085	0.52\\
0.00687560549718734	0.52\\
0.00687560549718734	0.53\\
0.00688041209843295	0.53\\
0.00688041209843295	0.54\\
0.00688322308744301	0.54\\
0.00688322308744301	0.55\\
0.00689341480763436	0.55\\
0.00689341480763436	0.56\\
0.00690180459866101	0.56\\
0.00690180459866101	0.57\\
0.00690631648921724	0.57\\
0.00690631648921724	0.58\\
0.00692350250255314	0.58\\
0.00692350250255314	0.59\\
0.00692415714623772	0.59\\
0.00692415714623772	0.6\\
0.00692706459492213	0.6\\
0.00692706459492213	0.61\\
0.00692811521293472	0.61\\
0.00692811521293472	0.62\\
0.00694132508060988	0.62\\
0.00694132508060988	0.63\\
0.00694747027538867	0.63\\
0.00694747027538867	0.64\\
0.00696447902670257	0.64\\
0.00696447902670257	0.65\\
0.00697885218236809	0.65\\
0.00697885218236809	0.66\\
0.00697998994538625	0.66\\
0.00697998994538625	0.67\\
0.00698089026183617	0.67\\
0.00698089026183617	0.68\\
0.00698886050575452	0.68\\
0.00698886050575452	0.69\\
0.00699347728704452	0.69\\
0.00699347728704452	0.7\\
0.00699445228160716	0.7\\
0.00699445228160716	0.71\\
0.00700024363357147	0.71\\
0.00700024363357147	0.72\\
0.00703515647796582	0.72\\
0.00703515647796582	0.73\\
0.00705293919011259	0.73\\
0.00705293919011259	0.74\\
0.00706666840442122	0.74\\
0.00706666840442122	0.75\\
0.00707374338173634	0.75\\
0.00707374338173634	0.76\\
0.00707935883172926	0.76\\
0.00707935883172926	0.77\\
0.00708973165635371	0.77\\
0.00708973165635371	0.78\\
0.00709033204312792	0.78\\
0.00709033204312792	0.79\\
0.00712502611020385	0.79\\
0.00712502611020385	0.8\\
0.00714302264006296	0.8\\
0.00714302264006296	0.81\\
0.00715106481882321	0.81\\
0.00715106481882321	0.82\\
0.00715558175162197	0.82\\
0.00715558175162197	0.83\\
0.00716296788994827	0.83\\
0.00716296788994827	0.84\\
0.0071717992877789	0.84\\
0.0071717992877789	0.85\\
0.00719582884520419	0.85\\
0.00719582884520419	0.86\\
0.00719978994612414	0.86\\
0.00719978994612414	0.87\\
0.00725214656916683	0.87\\
0.00725214656916683	0.88\\
0.0072559042471206	0.88\\
0.0072559042471206	0.89\\
0.00727206028014622	0.89\\
0.00727206028014622	0.9\\
0.0073002894567794	0.9\\
0.0073002894567794	0.91\\
0.00730865983457664	0.91\\
0.00730865983457664	0.92\\
0.00732552008791973	0.92\\
0.00732552008791973	0.93\\
0.00740587093370403	0.93\\
0.00740587093370403	0.94\\
0.00743721550781977	0.94\\
0.00743721550781977	0.95\\
0.00754312957575401	0.95\\
0.00754312957575401	0.96\\
0.00760432749786826	0.96\\
0.00760432749786826	0.97\\
0.00766434998081241	0.97\\
0.00766434998081241	0.98\\
0.00768174563188015	0.98\\
0.00768174563188015	0.99\\
0.00778197997001614	0.99\\
0.00778197997001614	1\\
inf	1\\
};
\addplot [color=mycolor4, forget plot,line width=1.5,dashed]
  table[row sep=crcr]{%
-inf	0\\
0.00011232224903237	0\\
0.00011232224903237	0.01\\
0.000132664259120409	0.01\\
0.000132664259120409	0.02\\
0.000135440705014567	0.02\\
0.000135440705014567	0.03\\
0.000137999779111252	0.03\\
0.000137999779111252	0.04\\
0.000139777631935138	0.04\\
0.000139777631935138	0.05\\
0.000144798553852591	0.05\\
0.000144798553852591	0.06\\
0.0001454215399217	0.06\\
0.0001454215399217	0.07\\
0.000146148071813339	0.07\\
0.000146148071813339	0.08\\
0.000151615712039857	0.08\\
0.000151615712039857	0.09\\
0.000152188939301633	0.09\\
0.000152188939301633	0.1\\
0.000153389718098912	0.1\\
0.000153389718098912	0.11\\
0.000155881877449653	0.11\\
0.000155881877449653	0.12\\
0.000159475196603521	0.12\\
0.000159475196603521	0.13\\
0.000162393021939165	0.13\\
0.000162393021939165	0.14\\
0.000162481736185424	0.14\\
0.000162481736185424	0.15\\
0.00016355839167028	0.15\\
0.00016355839167028	0.16\\
0.000164360212165144	0.16\\
0.000164360212165144	0.17\\
0.000166205628664413	0.17\\
0.000166205628664413	0.18\\
0.00016729967128035	0.18\\
0.00016729967128035	0.19\\
0.000167543972248635	0.19\\
0.000167543972248635	0.2\\
0.000168199159672017	0.2\\
0.000168199159672017	0.21\\
0.000168753160316601	0.21\\
0.000168753160316601	0.22\\
0.000170104066424328	0.22\\
0.000170104066424328	0.23\\
0.000171998178883475	0.23\\
0.000171998178883475	0.24\\
0.000172393757545375	0.24\\
0.000172393757545375	0.25\\
0.000172838328136889	0.25\\
0.000172838328136889	0.26\\
0.000173113337119311	0.26\\
0.000173113337119311	0.27\\
0.000173944450549086	0.27\\
0.000173944450549086	0.28\\
0.000175000527534652	0.28\\
0.000175000527534652	0.29\\
0.000175031242330986	0.29\\
0.000175031242330986	0.3\\
0.000175049882536907	0.3\\
0.000175049882536907	0.31\\
0.00017685385417011	0.31\\
0.00017685385417011	0.32\\
0.00017721340298952	0.32\\
0.00017721340298952	0.33\\
0.000178382725188189	0.33\\
0.000178382725188189	0.34\\
0.000179968888655554	0.34\\
0.000179968888655554	0.35\\
0.000180381275025027	0.35\\
0.000180381275025027	0.36\\
0.000182263019250601	0.36\\
0.000182263019250601	0.37\\
0.000184351631466098	0.37\\
0.000184351631466098	0.38\\
0.000185690609388068	0.38\\
0.000185690609388068	0.39\\
0.000185809971110344	0.39\\
0.000185809971110344	0.4\\
0.000186484144343535	0.4\\
0.000186484144343535	0.41\\
0.000186727973380558	0.41\\
0.000186727973380558	0.42\\
0.000187789617452051	0.42\\
0.000187789617452051	0.43\\
0.000190878716688063	0.43\\
0.000190878716688063	0.44\\
0.000192092391078644	0.44\\
0.000192092391078644	0.45\\
0.0001925708057419	0.45\\
0.0001925708057419	0.46\\
0.000192825329902341	0.46\\
0.000192825329902341	0.47\\
0.00019574668049318	0.47\\
0.00019574668049318	0.48\\
0.000196054427259001	0.48\\
0.000196054427259001	0.49\\
0.000196066120994377	0.49\\
0.000196066120994377	0.5\\
0.000196243712916713	0.5\\
0.000196243712916713	0.51\\
0.000197908542453539	0.51\\
0.000197908542453539	0.52\\
0.000199951866781676	0.52\\
0.000199951866781676	0.53\\
0.000201967012243252	0.53\\
0.000201967012243252	0.54\\
0.000204583495005922	0.54\\
0.000204583495005922	0.55\\
0.000205083620511362	0.55\\
0.000205083620511362	0.56\\
0.000206217822033662	0.56\\
0.000206217822033662	0.57\\
0.000210588176358721	0.57\\
0.000210588176358721	0.58\\
0.000210891628503493	0.58\\
0.000210891628503493	0.59\\
0.000211612889490476	0.59\\
0.000211612889490476	0.6\\
0.000216704452699321	0.6\\
0.000216704452699321	0.61\\
0.00021792486168125	0.61\\
0.00021792486168125	0.62\\
0.00021880506567007	0.62\\
0.00021880506567007	0.63\\
0.000220244805660615	0.63\\
0.000220244805660615	0.64\\
0.000223864472688557	0.64\\
0.000223864472688557	0.65\\
0.000225482117588474	0.65\\
0.000225482117588474	0.66\\
0.000235902796234541	0.66\\
0.000235902796234541	0.67\\
0.000236873568457471	0.67\\
0.000236873568457471	0.68\\
0.000238717174074063	0.68\\
0.000238717174074063	0.69\\
0.000240600914805742	0.69\\
0.000240600914805742	0.7\\
0.000242010799241503	0.7\\
0.000242010799241503	0.71\\
0.000248589256914538	0.71\\
0.000248589256914538	0.72\\
0.000248853053106988	0.72\\
0.000248853053106988	0.73\\
0.000249579117032489	0.73\\
0.000249579117032489	0.74\\
0.00025030545113763	0.74\\
0.00025030545113763	0.75\\
0.000251515601330918	0.75\\
0.000251515601330918	0.76\\
0.000255359436627307	0.76\\
0.000255359436627307	0.77\\
0.000255591279058822	0.77\\
0.000255591279058822	0.78\\
0.000257462691045095	0.78\\
0.000257462691045095	0.79\\
0.000259044884009224	0.79\\
0.000259044884009224	0.8\\
0.000263163762063586	0.8\\
0.000263163762063586	0.81\\
0.000265082226469375	0.81\\
0.000265082226469375	0.82\\
0.000270683907654262	0.82\\
0.000270683907654262	0.83\\
0.000271794779947823	0.83\\
0.000271794779947823	0.84\\
0.000274334055882935	0.84\\
0.000274334055882935	0.85\\
0.000275601789897137	0.85\\
0.000275601789897137	0.86\\
0.00027659085624157	0.86\\
0.00027659085624157	0.87\\
0.000276598188193763	0.87\\
0.000276598188193763	0.88\\
0.000279274580375057	0.88\\
0.000279274580375057	0.89\\
0.000284652041007721	0.89\\
0.000284652041007721	0.9\\
0.000289244724459333	0.9\\
0.000289244724459333	0.91\\
0.000294055228010513	0.91\\
0.000294055228010513	0.92\\
0.000295103004695487	0.92\\
0.000295103004695487	0.93\\
0.000301143470761249	0.93\\
0.000301143470761249	0.94\\
0.000306698642341025	0.94\\
0.000306698642341025	0.95\\
0.000309825544728867	0.95\\
0.000309825544728867	0.96\\
0.000312107851901522	0.96\\
0.000312107851901522	0.97\\
0.000317339375649714	0.97\\
0.000317339375649714	0.98\\
0.000352791213145002	0.98\\
0.000352791213145002	0.99\\
0.295800980029507	0.99\\
0.295800980029507	1\\
inf	1\\
};
\addplot [color=mycolor1, forget plot,line width=1.5]
  table[row sep=crcr]{%
-inf	0\\
0.00594100985237028	0\\
0.00594100985237028	0.01\\
0.00599009318527625	0.01\\
0.00599009318527625	0.02\\
0.00608293910923256	0.02\\
0.00608293910923256	0.03\\
0.00612100166685542	0.03\\
0.00612100166685542	0.04\\
0.0061438320642927	0.04\\
0.0061438320642927	0.05\\
0.00619205557790499	0.05\\
0.00619205557790499	0.06\\
0.00620959461818174	0.06\\
0.00620959461818174	0.07\\
0.00626229810250843	0.07\\
0.00626229810250843	0.08\\
0.00628484051723775	0.08\\
0.00628484051723775	0.09\\
0.00628787260249079	0.09\\
0.00628787260249079	0.1\\
0.00630051532259005	0.1\\
0.00630051532259005	0.11\\
0.00630513895786879	0.11\\
0.00630513895786879	0.12\\
0.00639814449263139	0.12\\
0.00639814449263139	0.13\\
0.00639999018185661	0.13\\
0.00639999018185661	0.14\\
0.00642100695036684	0.14\\
0.00642100695036684	0.15\\
0.0064223267240867	0.15\\
0.0064223267240867	0.16\\
0.00644484772732915	0.16\\
0.00644484772732915	0.17\\
0.00648379520670121	0.17\\
0.00648379520670121	0.18\\
0.00648595849995988	0.18\\
0.00648595849995988	0.19\\
0.0065160669128008	0.19\\
0.0065160669128008	0.2\\
0.00651800783203751	0.2\\
0.00651800783203751	0.21\\
0.00653780348947287	0.21\\
0.00653780348947287	0.22\\
0.00655071835161352	0.22\\
0.00655071835161352	0.23\\
0.00655097699606874	0.23\\
0.00655097699606874	0.24\\
0.00656035999919366	0.24\\
0.00656035999919366	0.25\\
0.00656521033430283	0.25\\
0.00656521033430283	0.26\\
0.00656770409220368	0.26\\
0.00656770409220368	0.27\\
0.00657314285487407	0.27\\
0.00657314285487407	0.28\\
0.00660724824334752	0.28\\
0.00660724824334752	0.29\\
0.00661443603215063	0.29\\
0.00661443603215063	0.3\\
0.00661949165534638	0.3\\
0.00661949165534638	0.31\\
0.00662172939798818	0.31\\
0.00662172939798818	0.32\\
0.0066234818202168	0.32\\
0.0066234818202168	0.33\\
0.00663655304330502	0.33\\
0.00663655304330502	0.34\\
0.00666537258185465	0.34\\
0.00666537258185465	0.35\\
0.00666997356377142	0.35\\
0.00666997356377142	0.36\\
0.00668990634013947	0.36\\
0.00668990634013947	0.37\\
0.00669850296160555	0.37\\
0.00669850296160555	0.38\\
0.00672666207867346	0.38\\
0.00672666207867346	0.39\\
0.00672793821785664	0.39\\
0.00672793821785664	0.4\\
0.00673900999319645	0.4\\
0.00673900999319645	0.41\\
0.0067480603076519	0.41\\
0.0067480603076519	0.42\\
0.00679255448276614	0.42\\
0.00679255448276614	0.43\\
0.00680142826592546	0.43\\
0.00680142826592546	0.44\\
0.00680652403559258	0.44\\
0.00680652403559258	0.45\\
0.0068112915584925	0.45\\
0.0068112915584925	0.46\\
0.0068114050883781	0.46\\
0.0068114050883781	0.47\\
0.00681325895554897	0.47\\
0.00681325895554897	0.48\\
0.00682774836370451	0.48\\
0.00682774836370451	0.49\\
0.00682867776816079	0.49\\
0.00682867776816079	0.5\\
0.00686081372727172	0.5\\
0.00686081372727172	0.51\\
0.00687319130309085	0.51\\
0.00687319130309085	0.52\\
0.00687560549718734	0.52\\
0.00687560549718734	0.53\\
0.00688041209843295	0.53\\
0.00688041209843295	0.54\\
0.00688322308744301	0.54\\
0.00688322308744301	0.55\\
0.00689341480763436	0.55\\
0.00689341480763436	0.56\\
0.00690180459866101	0.56\\
0.00690180459866101	0.57\\
0.00690631648921724	0.57\\
0.00690631648921724	0.58\\
0.00692350250255314	0.58\\
0.00692350250255314	0.59\\
0.00692415714623772	0.59\\
0.00692415714623772	0.6\\
0.00692706459492213	0.6\\
0.00692706459492213	0.61\\
0.00692811521293472	0.61\\
0.00692811521293472	0.62\\
0.00694132508060988	0.62\\
0.00694132508060988	0.63\\
0.00694747027538867	0.63\\
0.00694747027538867	0.64\\
0.00696447902670257	0.64\\
0.00696447902670257	0.65\\
0.00697885218236809	0.65\\
0.00697885218236809	0.66\\
0.00697998994538625	0.66\\
0.00697998994538625	0.67\\
0.00698089026183617	0.67\\
0.00698089026183617	0.68\\
0.00698886050575452	0.68\\
0.00698886050575452	0.69\\
0.00699347728704452	0.69\\
0.00699347728704452	0.7\\
0.00699445228160716	0.7\\
0.00699445228160716	0.71\\
0.00700024363357147	0.71\\
0.00700024363357147	0.72\\
0.00703515647796582	0.72\\
0.00703515647796582	0.73\\
0.00705293919011259	0.73\\
0.00705293919011259	0.74\\
0.00706666840442122	0.74\\
0.00706666840442122	0.75\\
0.00707374338173634	0.75\\
0.00707374338173634	0.76\\
0.00707935883172926	0.76\\
0.00707935883172926	0.77\\
0.00708973165635371	0.77\\
0.00708973165635371	0.78\\
0.00709033204312792	0.78\\
0.00709033204312792	0.79\\
0.00712502611020385	0.79\\
0.00712502611020385	0.8\\
0.00714302264006296	0.8\\
0.00714302264006296	0.81\\
0.00715106481882321	0.81\\
0.00715106481882321	0.82\\
0.00715558175162197	0.82\\
0.00715558175162197	0.83\\
0.00716296788994827	0.83\\
0.00716296788994827	0.84\\
0.0071717992877789	0.84\\
0.0071717992877789	0.85\\
0.00719582884520419	0.85\\
0.00719582884520419	0.86\\
0.00719978994612414	0.86\\
0.00719978994612414	0.87\\
0.00725214656916683	0.87\\
0.00725214656916683	0.88\\
0.0072559042471206	0.88\\
0.0072559042471206	0.89\\
0.00727206028014622	0.89\\
0.00727206028014622	0.9\\
0.0073002894567794	0.9\\
0.0073002894567794	0.91\\
0.00730865983457664	0.91\\
0.00730865983457664	0.92\\
0.00732552008791973	0.92\\
0.00732552008791973	0.93\\
0.00740587093370403	0.93\\
0.00740587093370403	0.94\\
0.00743721550781977	0.94\\
0.00743721550781977	0.95\\
0.00754312957575401	0.95\\
0.00754312957575401	0.96\\
0.00760432749786826	0.96\\
0.00760432749786826	0.97\\
0.00766434998081241	0.97\\
0.00766434998081241	0.98\\
0.00768174563188015	0.98\\
0.00768174563188015	0.99\\
0.00778197997001614	0.99\\
0.00778197997001614	1\\
inf	1\\
};
\addplot [color=mycolor4, forget plot,line width=1.5,dashed]
  table[row sep=crcr]{%
-inf	0\\
0.00011232224903237	0\\
0.00011232224903237	0.01\\
0.000132664259120409	0.01\\
0.000132664259120409	0.02\\
0.000135440705014567	0.02\\
0.000135440705014567	0.03\\
0.000137999779111252	0.03\\
0.000137999779111252	0.04\\
0.000139777631935138	0.04\\
0.000139777631935138	0.05\\
0.000144798553852591	0.05\\
0.000144798553852591	0.06\\
0.0001454215399217	0.06\\
0.0001454215399217	0.07\\
0.000146148071813339	0.07\\
0.000146148071813339	0.08\\
0.000151615712039857	0.08\\
0.000151615712039857	0.09\\
0.000152188939301633	0.09\\
0.000152188939301633	0.1\\
0.000153389718098912	0.1\\
0.000153389718098912	0.11\\
0.000155881877449653	0.11\\
0.000155881877449653	0.12\\
0.000159475196603521	0.12\\
0.000159475196603521	0.13\\
0.000162393021939165	0.13\\
0.000162393021939165	0.14\\
0.000162481736185424	0.14\\
0.000162481736185424	0.15\\
0.00016355839167028	0.15\\
0.00016355839167028	0.16\\
0.000164360212165144	0.16\\
0.000164360212165144	0.17\\
0.000166205628664413	0.17\\
0.000166205628664413	0.18\\
0.00016729967128035	0.18\\
0.00016729967128035	0.19\\
0.000167543972248635	0.19\\
0.000167543972248635	0.2\\
0.000168199159672017	0.2\\
0.000168199159672017	0.21\\
0.000168753160316601	0.21\\
0.000168753160316601	0.22\\
0.000170104066424328	0.22\\
0.000170104066424328	0.23\\
0.000171998178883475	0.23\\
0.000171998178883475	0.24\\
0.000172393757545375	0.24\\
0.000172393757545375	0.25\\
0.000172838328136889	0.25\\
0.000172838328136889	0.26\\
0.000173113337119311	0.26\\
0.000173113337119311	0.27\\
0.000173944450549086	0.27\\
0.000173944450549086	0.28\\
0.000175000527534652	0.28\\
0.000175000527534652	0.29\\
0.000175031242330986	0.29\\
0.000175031242330986	0.3\\
0.000175049882536907	0.3\\
0.000175049882536907	0.31\\
0.00017685385417011	0.31\\
0.00017685385417011	0.32\\
0.00017721340298952	0.32\\
0.00017721340298952	0.33\\
0.000178382725188189	0.33\\
0.000178382725188189	0.34\\
0.000179968888655554	0.34\\
0.000179968888655554	0.35\\
0.000180381275025027	0.35\\
0.000180381275025027	0.36\\
0.000182263019250601	0.36\\
0.000182263019250601	0.37\\
0.000184351631466098	0.37\\
0.000184351631466098	0.38\\
0.000185690609388068	0.38\\
0.000185690609388068	0.39\\
0.000185809971110344	0.39\\
0.000185809971110344	0.4\\
0.000186484144343535	0.4\\
0.000186484144343535	0.41\\
0.000186727973380558	0.41\\
0.000186727973380558	0.42\\
0.000187789617452051	0.42\\
0.000187789617452051	0.43\\
0.000190878716688063	0.43\\
0.000190878716688063	0.44\\
0.000192092391078644	0.44\\
0.000192092391078644	0.45\\
0.0001925708057419	0.45\\
0.0001925708057419	0.46\\
0.000192825329902341	0.46\\
0.000192825329902341	0.47\\
0.00019574668049318	0.47\\
0.00019574668049318	0.48\\
0.000196054427259001	0.48\\
0.000196054427259001	0.49\\
0.000196066120994377	0.49\\
0.000196066120994377	0.5\\
0.000196243712916713	0.5\\
0.000196243712916713	0.51\\
0.000197908542453539	0.51\\
0.000197908542453539	0.52\\
0.000199951866781676	0.52\\
0.000199951866781676	0.53\\
0.000201967012243252	0.53\\
0.000201967012243252	0.54\\
0.000204583495005922	0.54\\
0.000204583495005922	0.55\\
0.000205083620511362	0.55\\
0.000205083620511362	0.56\\
0.000206217822033662	0.56\\
0.000206217822033662	0.57\\
0.000210588176358721	0.57\\
0.000210588176358721	0.58\\
0.000210891628503493	0.58\\
0.000210891628503493	0.59\\
0.000211612889490476	0.59\\
0.000211612889490476	0.6\\
0.000216704452699321	0.6\\
0.000216704452699321	0.61\\
0.00021792486168125	0.61\\
0.00021792486168125	0.62\\
0.00021880506567007	0.62\\
0.00021880506567007	0.63\\
0.000220244805660615	0.63\\
0.000220244805660615	0.64\\
0.000223864472688557	0.64\\
0.000223864472688557	0.65\\
0.000225482117588474	0.65\\
0.000225482117588474	0.66\\
0.000235902796234541	0.66\\
0.000235902796234541	0.67\\
0.000236873568457471	0.67\\
0.000236873568457471	0.68\\
0.000238717174074063	0.68\\
0.000238717174074063	0.69\\
0.000240600914805742	0.69\\
0.000240600914805742	0.7\\
0.000242010799241503	0.7\\
0.000242010799241503	0.71\\
0.000248589256914538	0.71\\
0.000248589256914538	0.72\\
0.000248853053106988	0.72\\
0.000248853053106988	0.73\\
0.000249579117032489	0.73\\
0.000249579117032489	0.74\\
0.00025030545113763	0.74\\
0.00025030545113763	0.75\\
0.000251515601330918	0.75\\
0.000251515601330918	0.76\\
0.000255359436627307	0.76\\
0.000255359436627307	0.77\\
0.000255591279058822	0.77\\
0.000255591279058822	0.78\\
0.000257462691045095	0.78\\
0.000257462691045095	0.79\\
0.000259044884009224	0.79\\
0.000259044884009224	0.8\\
0.000263163762063586	0.8\\
0.000263163762063586	0.81\\
0.000265082226469375	0.81\\
0.000265082226469375	0.82\\
0.000270683907654262	0.82\\
0.000270683907654262	0.83\\
0.000271794779947823	0.83\\
0.000271794779947823	0.84\\
0.000274334055882935	0.84\\
0.000274334055882935	0.85\\
0.000275601789897137	0.85\\
0.000275601789897137	0.86\\
0.00027659085624157	0.86\\
0.00027659085624157	0.87\\
0.000276598188193763	0.87\\
0.000276598188193763	0.88\\
0.000279274580375057	0.88\\
0.000279274580375057	0.89\\
0.000284652041007721	0.89\\
0.000284652041007721	0.9\\
0.000289244724459333	0.9\\
0.000289244724459333	0.91\\
0.000294055228010513	0.91\\
0.000294055228010513	0.92\\
0.000295103004695487	0.92\\
0.000295103004695487	0.93\\
0.000301143470761249	0.93\\
0.000301143470761249	0.94\\
0.000306698642341025	0.94\\
0.000306698642341025	0.95\\
0.000309825544728867	0.95\\
0.000309825544728867	0.96\\
0.000312107851901522	0.96\\
0.000312107851901522	0.97\\
0.000317339375649714	0.97\\
0.000317339375649714	0.98\\
0.000352791213145002	0.98\\
0.000352791213145002	0.99\\
0.295800980029507	0.99\\
0.295800980029507	1\\
inf	1\\
};
\addplot [color=mycolor3, forget plot,line width=1.5]
  table[row sep=crcr]{%
-inf	0\\
0.000169451932988865	0\\
0.000169451932988865	0.01\\
0.000170869657332569	0.01\\
0.000170869657332569	0.02\\
0.000173156469361578	0.02\\
0.000173156469361578	0.03\\
0.000174930582071079	0.03\\
0.000174930582071079	0.04\\
0.000176567069641178	0.04\\
0.000176567069641178	0.05\\
0.000177092734381889	0.05\\
0.000177092734381889	0.06\\
0.000178180324037252	0.06\\
0.000178180324037252	0.07\\
0.000178739405469641	0.07\\
0.000178739405469641	0.08\\
0.000178782934322459	0.08\\
0.000178782934322459	0.09\\
0.000179225418848838	0.09\\
0.000179225418848838	0.1\\
0.00017936980249678	0.1\\
0.00017936980249678	0.11\\
0.000179690545128542	0.11\\
0.000179690545128542	0.12\\
0.000181061753011422	0.12\\
0.000181061753011422	0.13\\
0.000181315210818848	0.13\\
0.000181315210818848	0.14\\
0.000182595537689047	0.14\\
0.000182595537689047	0.15\\
0.000183208590238391	0.15\\
0.000183208590238391	0.16\\
0.000183695248950714	0.16\\
0.000183695248950714	0.17\\
0.000183759674345899	0.17\\
0.000183759674345899	0.18\\
0.000184069244218566	0.18\\
0.000184069244218566	0.19\\
0.000184594198040962	0.19\\
0.000184594198040962	0.2\\
0.000186004387195599	0.2\\
0.000186004387195599	0.21\\
0.000186072700172296	0.21\\
0.000186072700172296	0.22\\
0.000186418358382107	0.22\\
0.000186418358382107	0.23\\
0.000187648663810391	0.23\\
0.000187648663810391	0.24\\
0.000189327266663453	0.24\\
0.000189327266663453	0.25\\
0.00019040945629639	0.25\\
0.00019040945629639	0.26\\
0.000191068345025673	0.26\\
0.000191068345025673	0.27\\
0.000191305308792704	0.27\\
0.000191305308792704	0.28\\
0.000192501150514091	0.28\\
0.000192501150514091	0.29\\
0.000192722218123993	0.29\\
0.000192722218123993	0.3\\
0.000193626695705274	0.3\\
0.000193626695705274	0.31\\
0.000194419278937604	0.31\\
0.000194419278937604	0.32\\
0.000194597724918652	0.32\\
0.000194597724918652	0.33\\
0.000194890336433903	0.33\\
0.000194890336433903	0.34\\
0.000195886119089187	0.34\\
0.000195886119089187	0.35\\
0.000197398180765593	0.35\\
0.000197398180765593	0.36\\
0.000197642912999712	0.36\\
0.000197642912999712	0.37\\
0.000198134754562639	0.37\\
0.000198134754562639	0.38\\
0.000198211078143339	0.38\\
0.000198211078143339	0.39\\
0.000199969031674611	0.39\\
0.000199969031674611	0.4\\
0.000200471637934734	0.4\\
0.000200471637934734	0.41\\
0.000200778820591404	0.41\\
0.000200778820591404	0.42\\
0.000200966776759283	0.42\\
0.000200966776759283	0.43\\
0.000201051526602986	0.43\\
0.000201051526602986	0.44\\
0.000202693726358974	0.44\\
0.000202693726358974	0.45\\
0.000203331707488145	0.45\\
0.000203331707488145	0.46\\
0.000203629403148983	0.46\\
0.000203629403148983	0.47\\
0.000203955028517735	0.47\\
0.000203955028517735	0.48\\
0.000205639339371028	0.48\\
0.000205639339371028	0.49\\
0.000207847061506499	0.49\\
0.000207847061506499	0.5\\
0.00021305485584712	0.5\\
0.00021305485584712	0.51\\
0.000213061313424855	0.51\\
0.000213061313424855	0.52\\
0.000213984108915761	0.52\\
0.000213984108915761	0.53\\
0.000215250908037233	0.53\\
0.000215250908037233	0.54\\
0.000215264494991469	0.54\\
0.000215264494991469	0.55\\
0.00021611685383286	0.55\\
0.00021611685383286	0.56\\
0.000218414461217534	0.56\\
0.000218414461217534	0.57\\
0.000218510731902112	0.57\\
0.000218510731902112	0.58\\
0.000220054823579761	0.58\\
0.000220054823579761	0.59\\
0.000220462096759053	0.59\\
0.000220462096759053	0.6\\
0.00022091241256949	0.6\\
0.00022091241256949	0.61\\
0.000221304140312445	0.61\\
0.000221304140312445	0.62\\
0.000222442056363868	0.62\\
0.000222442056363868	0.63\\
0.000223730765778116	0.63\\
0.000223730765778116	0.64\\
0.000225108971793075	0.64\\
0.000225108971793075	0.65\\
0.00022650347862618	0.65\\
0.00022650347862618	0.66\\
0.000228064338606816	0.66\\
0.000228064338606816	0.67\\
0.000229180995349608	0.67\\
0.000229180995349608	0.68\\
0.00022946257084252	0.68\\
0.00022946257084252	0.69\\
0.000229884808400469	0.69\\
0.000229884808400469	0.7\\
0.000230741162581845	0.7\\
0.000230741162581845	0.71\\
0.000231019748245648	0.71\\
0.000231019748245648	0.72\\
0.000231063652675362	0.72\\
0.000231063652675362	0.73\\
0.000233995913554055	0.73\\
0.000233995913554055	0.74\\
0.000241289868582132	0.74\\
0.000241289868582132	0.75\\
0.000241471595774144	0.75\\
0.000241471595774144	0.76\\
0.000242252936494447	0.76\\
0.000242252936494447	0.77\\
0.000242539790876054	0.77\\
0.000242539790876054	0.78\\
0.000242875602992037	0.78\\
0.000242875602992037	0.79\\
0.000244766266441542	0.79\\
0.000244766266441542	0.8\\
0.000246993918881895	0.8\\
0.000246993918881895	0.81\\
0.000248131826193716	0.81\\
0.000248131826193716	0.82\\
0.000249004126418729	0.82\\
0.000249004126418729	0.83\\
0.000251662570457004	0.83\\
0.000251662570457004	0.84\\
0.000253209340812731	0.84\\
0.000253209340812731	0.85\\
0.000254596684461822	0.85\\
0.000254596684461822	0.86\\
0.000254789408126122	0.86\\
0.000254789408126122	0.87\\
0.000256474968321403	0.87\\
0.000256474968321403	0.88\\
0.000257033885416166	0.88\\
0.000257033885416166	0.89\\
0.000262301382543647	0.89\\
0.000262301382543647	0.9\\
0.000264877487134934	0.9\\
0.000264877487134934	0.91\\
0.000270757241380963	0.91\\
0.000270757241380963	0.92\\
0.000281336069929461	0.92\\
0.000281336069929461	0.93\\
0.000290909833815923	0.93\\
0.000290909833815923	0.94\\
0.000292632780932241	0.94\\
0.000292632780932241	0.95\\
0.000312570101551869	0.95\\
0.000312570101551869	0.96\\
0.000335229906777619	0.96\\
0.000335229906777619	0.97\\
0.000338043068859436	0.97\\
0.000338043068859436	0.98\\
0.000357779962321375	0.98\\
0.000357779962321375	0.99\\
0.00043819838807345	0.99\\
0.00043819838807345	1\\
inf	1\\
};
\end{axis}


==> RIS-Enabled Personal Radar/pebs.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
\definecolor{mycolor1}{rgb}{0.00000,0.44700,0.74100}%
\definecolor{mycolor2}{rgb}{0.85000,0.32500,0.09800}%
\definecolor{mycolor3}{rgb}{0.92900,0.69400,0.12500}%
\definecolor{mycolor4}{rgb}{0.49400,0.18400,0.55600}%
%

\begin{axis}[%
at={(-2.1cm,0cm)},
width=4.5cm,
height=4cm,
scale only axis,
xmode=log,
xmin=1,
xmax=50,
xminorticks=true,
ymode=log,
ymin=1e-05,
ymax=1,
yminorticks=true,
xlabel={\footnotesize a) $d [\mathrm{m}] $},
axis background/.style={fill=white},
axis x line*=bottom,
axis y line*=left,
xmajorgrids,
xminorgrids,
ymajorgrids
]
\node[rotate=40,fill=white] at (axis cs:5,.002) {\footnotesize Random };
\node[rotate=40,fill=white] at (axis cs:5,.0001) {\footnotesize Directional };
\draw (axis cs:5.5,.00004) ellipse (.1cm and .2cm);
\draw (axis cs:5,.0005) ellipse (.1cm and .2cm);
\addplot [color=mycolor1, forget plot,line width=1.5]
  table[row sep=crcr]{%
1	6.63281576565766e-06\\
1.27427498570313	1.24571876487842e-05\\
1.62377673918872	2.36650160410122e-05\\
2.06913808111479	4.62631554608735e-05\\
2.63665089873036	9.21629543630577e-05\\
3.35981828628378	0.000183484676614509\\
4.28133239871939	0.00037425910813291\\
5.45559478116852	0.00077568945676615\\
6.95192796177561	0.00159952316003032\\
8.85866790410082	0.00328525775217572\\
11.2883789168469	0.00682172379372616\\
14.3844988828766	0.013979385767212\\
18.3298071083244	0.0291163506771437\\
23.3572146909012	0.0597000312530902\\
29.7635144163132	0.124474080972064\\
37.9269019073225	0.255889550119898\\
48.3293023857175	0.533321161619385\\
61.5848211066026	1.08915903729389\\
78.4759970351461	2.25149374807732\\
100	4.71593981321998\\
};
\addplot [color=mycolor2, only marks, mark=square, mark options={solid, mycolor2}, forget plot,line width=1.5]
  table[row sep=crcr]{%
1	6.72279038578006e-06\\
1.27427498570313	1.23268703824158e-05\\
1.62377673918872	2.38731891207223e-05\\
2.06913808111479	4.57529020429913e-05\\
2.63665089873036	9.31246022913377e-05\\
3.35981828628378	0.000176224624070884\\
4.28133239871939	0.000376478356951156\\
5.45559478116852	0.000769662324158172\\
6.95192796177561	0.00156175716162269\\
8.85866790410082	0.00318097867570969\\
11.2883789168469	0.0067711843946802\\
14.3844988828766	0.0136858058334389\\
18.3298071083244	0.0293652801743878\\
23.3572146909012	28.7318112776332\\
29.7635144163132	65.9973667580549\\
37.9269019073225	69.542719287805\\
48.3293023857175	72.9168174196587\\
61.5848211066026	76.5911097870799\\
78.4759970351461	88.4599553841714\\
100	103.861753045388\\
};
\addplot [color=mycolor3, forget plot,line width=1.5]
  table[row sep=crcr]{%
1	1.12338936370682e-06\\
1.27427498570313	1.87460475005799e-06\\
1.62377673918872	3.04668160942692e-06\\
2.06913808111479	5.37682295309639e-06\\
2.63665089873036	7.92093407968065e-06\\
3.35981828628378	1.38186206893606e-05\\
4.28133239871939	2.49360077906243e-05\\
5.45559478116852	3.76186644506405e-05\\
6.95192796177561	6.33526113773838e-05\\
8.85866790410082	0.000116867060560047\\
11.2883789168469	0.000219882940076596\\
14.3844988828766	0.000454581110384452\\
18.3298071083244	0.00100513740943559\\
23.3572146909012	0.00229589529818709\\
29.7635144163132	0.00559073226515006\\
37.9269019073225	0.0139645885520947\\
48.3293023857175	0.0360221369647204\\
61.5848211066026	0.092204881974793\\
78.4759970351461	0.235965991138321\\
100	0.625172892276431\\
};
\addplot [color=mycolor4, only marks, mark=x, mark options={solid, mycolor4}, forget plot,line width=1.5]
  table[row sep=crcr]{%
1	1.38221325018614e-06\\
1.27427498570313	1.88643231719039e-06\\
1.62377673918872	2.92255144284642e-06\\
2.06913808111479	5.22366805894463e-06\\
2.63665089873036	7.85622834184143e-06\\
3.35981828628378	1.39019470310631e-05\\
4.28133239871939	2.50691962286822e-05\\
5.45559478116852	3.68332357706635e-05\\
6.95192796177561	6.11612065231306e-05\\
8.85866790410082	0.00011617731638305\\
11.2883789168469	0.00316621090381372\\
14.3844988828766	0.000453233372436663\\
18.3298071083244	0.000985942686187251\\
23.3572146909012	0.00222292747353848\\
29.7635144163132	0.00548669383919826\\
37.9269019073225	0.726807941102239\\
48.3293023857175	19.1536801881545\\
61.5848211066026	37.7014872059233\\
78.4759970351461	60.477604664735\\
100	87.1948210503601\\
};
\end{axis}


==> cdfs.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
%\definecolor{mycolor1}{rgb}{0.00000,0.44700,0.74100}%
%\definecolor{mycolor2}{rgb}{0.85000,0.32500,0.09800}%
%

\begin{axis}[%
at={(3.5cm,0)},
width=4.5cm,
height=4cm,
scale only axis,
unbounded coords=jump,
xmode=log,
xmin=1e-4,
xmax=0.03,
xminorticks=true,
xlabel style={font=\color{white!15!black}},
xlabel={\footnotesize $b) e[\mathrm{m}]$},
ymin=0,
ymax=1,
axis background/.style={fill=white},
title style={font=\bfseries},
axis x line*=bottom,
axis y line*=left,
xmajorgrids,
xminorgrids,
ymajorgrids
]
\node[rotate=0,fill=white] at (axis cs:.003,.6) {\footnotesize Random};
\node[rotate=0,fill=white] at (axis cs:.0006,.5) {\footnotesize Directional};
\draw (axis cs:.007,.6) ellipse (.2cm and .1cm);
\draw (axis cs:.0002,.5) ellipse (.2cm and .1cm);
\addplot [color=mycolor2, forget plot,line width=1.5,dashed]
  table[row sep=crcr]{%
-inf	0\\
0.00388763495332524	0\\
0.00388763495332524	0.01\\
0.0039779769369078	0.01\\
0.0039779769369078	0.02\\
0.00437702219895772	0.02\\
0.00437702219895772	0.03\\
0.0045279377194668	0.03\\
0.0045279377194668	0.04\\
0.00456982329175554	0.04\\
0.00456982329175554	0.05\\
0.00483098405479953	0.05\\
0.00483098405479953	0.06\\
0.00494256970577131	0.06\\
0.00494256970577131	0.07\\
0.00501030301268805	0.07\\
0.00501030301268805	0.08\\
0.00513783394341532	0.08\\
0.00513783394341532	0.09\\
0.00519586445469606	0.09\\
0.00519586445469606	0.1\\
0.00523357784167244	0.1\\
0.00523357784167244	0.11\\
0.00525944393745265	0.11\\
0.00525944393745265	0.12\\
0.00531603796773738	0.12\\
0.00531603796773738	0.13\\
0.00541826257025269	0.13\\
0.00541826257025269	0.14\\
0.00543579830221148	0.14\\
0.00543579830221148	0.15\\
0.00547540416269369	0.15\\
0.00547540416269369	0.16\\
0.0054851530725855	0.16\\
0.0054851530725855	0.17\\
0.00550140659815427	0.17\\
0.00550140659815427	0.18\\
0.00552060998763975	0.18\\
0.00552060998763975	0.19\\
0.00555979050277402	0.19\\
0.00555979050277402	0.2\\
0.00556285059006915	0.2\\
0.00556285059006915	0.21\\
0.00568453435581969	0.21\\
0.00568453435581969	0.22\\
0.00569204200507351	0.22\\
0.00569204200507351	0.23\\
0.00579280694758293	0.23\\
0.00579280694758293	0.24\\
0.00579995431037703	0.24\\
0.00579995431037703	0.25\\
0.00588773873775303	0.25\\
0.00588773873775303	0.26\\
0.00593842205392088	0.26\\
0.00593842205392088	0.27\\
0.00603254823975779	0.27\\
0.00603254823975779	0.28\\
0.00612865636514691	0.28\\
0.00612865636514691	0.29\\
0.0061630099478404	0.29\\
0.0061630099478404	0.3\\
0.00617432934146672	0.3\\
0.00617432934146672	0.31\\
0.00618994226040939	0.31\\
0.00618994226040939	0.32\\
0.00620976839154533	0.32\\
0.00620976839154533	0.33\\
0.00621589041047224	0.33\\
0.00621589041047224	0.34\\
0.00622299644651732	0.34\\
0.00622299644651732	0.35\\
0.0062343259165862	0.35\\
0.0062343259165862	0.36\\
0.00627648039045602	0.36\\
0.00627648039045602	0.37\\
0.00634545501416627	0.37\\
0.00634545501416627	0.38\\
0.00637730768160198	0.38\\
0.00637730768160198	0.39\\
0.00640788564009761	0.39\\
0.00640788564009761	0.4\\
0.006415855404117	0.4\\
0.006415855404117	0.41\\
0.00646372169868585	0.41\\
0.00646372169868585	0.42\\
0.00654699862180399	0.42\\
0.00654699862180399	0.43\\
0.00656728063394036	0.43\\
0.00656728063394036	0.44\\
0.00658800268562385	0.44\\
0.00658800268562385	0.45\\
0.00661947482080476	0.45\\
0.00661947482080476	0.46\\
0.00671287872309909	0.46\\
0.00671287872309909	0.47\\
0.00673209634434497	0.47\\
0.00673209634434497	0.48\\
0.00673873996814358	0.48\\
0.00673873996814358	0.49\\
0.00676493352657311	0.49\\
0.00676493352657311	0.5\\
0.00678293182547686	0.5\\
0.00678293182547686	0.51\\
0.0067864636826908	0.51\\
0.0067864636826908	0.52\\
0.00688843352181448	0.52\\
0.00688843352181448	0.53\\
0.00690218623404389	0.53\\
0.00690218623404389	0.54\\
0.00692059412019435	0.54\\
0.00692059412019435	0.55\\
0.00695228513937172	0.55\\
0.00695228513937172	0.56\\
0.00696268765805748	0.56\\
0.00696268765805748	0.57\\
0.00698901995086007	0.57\\
0.00698901995086007	0.58\\
0.00701887482569471	0.58\\
0.00701887482569471	0.59\\
0.0070881888437203	0.59\\
0.0070881888437203	0.6\\
0.00709133457158546	0.6\\
0.00709133457158546	0.61\\
0.00709938665983232	0.61\\
0.00709938665983232	0.62\\
0.0071103192620758	0.62\\
0.0071103192620758	0.63\\
0.00714802314516168	0.63\\
0.00714802314516168	0.64\\
0.00717948379555864	0.64\\
0.00717948379555864	0.65\\
0.00720661799340744	0.65\\
0.00720661799340744	0.66\\
0.00721072490628053	0.66\\
0.00721072490628053	0.67\\
0.00727713275796887	0.67\\
0.00727713275796887	0.68\\
0.00733014380839564	0.68\\
0.00733014380839564	0.69\\
0.00734040335966124	0.69\\
0.00734040335966124	0.7\\
0.00736378800319066	0.7\\
0.00736378800319066	0.71\\
0.00736572374519651	0.71\\
0.00736572374519651	0.72\\
0.0073765123257748	0.72\\
0.0073765123257748	0.73\\
0.00741673477843082	0.73\\
0.00741673477843082	0.74\\
0.00749952340862622	0.74\\
0.00749952340862622	0.75\\
0.00753265357893415	0.75\\
0.00753265357893415	0.76\\
0.00754037977442961	0.76\\
0.00754037977442961	0.77\\
0.00758943452362781	0.77\\
0.00758943452362781	0.78\\
0.00761475721000997	0.78\\
0.00761475721000997	0.79\\
0.0077412746042716	0.79\\
0.0077412746042716	0.8\\
0.00776843123485257	0.8\\
0.00776843123485257	0.81\\
0.00783275913583604	0.81\\
0.00783275913583604	0.82\\
0.00791905001768998	0.82\\
0.00791905001768998	0.83\\
0.00807806751081398	0.83\\
0.00807806751081398	0.84\\
0.00813986797387923	0.84\\
0.00813986797387923	0.85\\
0.00825723615635137	0.85\\
0.00825723615635137	0.86\\
0.0082713869507189	0.86\\
0.0082713869507189	0.87\\
0.00831161454742953	0.87\\
0.00831161454742953	0.88\\
0.00851917175990109	0.88\\
0.00851917175990109	0.89\\
0.0085322476072092	0.89\\
0.0085322476072092	0.9\\
0.00861277743903294	0.9\\
0.00861277743903294	0.91\\
0.00865109615772425	0.91\\
0.00865109615772425	0.92\\
0.00872005431699495	0.92\\
0.00872005431699495	0.93\\
0.00872265152206257	0.93\\
0.00872265152206257	0.94\\
0.00880711469000858	0.94\\
0.00880711469000858	0.95\\
0.00888147476122421	0.95\\
0.00888147476122421	0.96\\
0.00943840673278368	0.96\\
0.00943840673278368	0.97\\
0.00945555000782478	0.97\\
0.00945555000782478	0.98\\
0.00978202883359448	0.98\\
0.00978202883359448	0.99\\
0.00994107140898879	0.99\\
0.00994107140898879	1\\
inf	1\\
};
\node[rotate=0,fill=white] at (axis cs:.0006,.5) {\footnotesize Directional};
\draw (axis cs:.007,.6) ellipse (.2cm and .1cm);
\draw (axis cs:.0002,.5) ellipse (.2cm and .1cm);
\addplot [color=mycolor2, forget plot,line width=1.5,dashed]
  table[row sep=crcr]{%
-inf	0\\
0.00388763495332524	0\\
0.00388763495332524	0.01\\
0.0039779769369078	0.01\\
0.0039779769369078	0.02\\
0.00437702219895772	0.02\\
0.00437702219895772	0.03\\
0.0045279377194668	0.03\\
0.0045279377194668	0.04\\
0.00456982329175554	0.04\\
0.00456982329175554	0.05\\
0.00483098405479953	0.05\\
0.00483098405479953	0.06\\
0.00494256970577131	0.06\\
0.00494256970577131	0.07\\
0.00501030301268805	0.07\\
0.00501030301268805	0.08\\
0.00513783394341532	0.08\\
0.00513783394341532	0.09\\
0.00519586445469606	0.09\\
0.00519586445469606	0.1\\
0.00523357784167244	0.1\\
0.00523357784167244	0.11\\
0.00525944393745265	0.11\\
0.00525944393745265	0.12\\
0.00531603796773738	0.12\\
0.00531603796773738	0.13\\
0.00541826257025269	0.13\\
0.00541826257025269	0.14\\
0.00543579830221148	0.14\\
0.00543579830221148	0.15\\
0.00547540416269369	0.15\\
0.00547540416269369	0.16\\
0.0054851530725855	0.16\\
0.0054851530725855	0.17\\
0.00550140659815427	0.17\\
0.00550140659815427	0.18\\
0.00552060998763975	0.18\\
0.00552060998763975	0.19\\
0.00555979050277402	0.19\\
0.00555979050277402	0.2\\
0.00556285059006915	0.2\\
0.00556285059006915	0.21\\
0.00568453435581969	0.21\\
0.00568453435581969	0.22\\
0.00569204200507351	0.22\\
0.00569204200507351	0.23\\
0.00579280694758293	0.23\\
0.00579280694758293	0.24\\
0.00579995431037703	0.24\\
0.00579995431037703	0.25\\
0.00588773873775303	0.25\\
0.00588773873775303	0.26\\
0.00593842205392088	0.26\\
0.00593842205392088	0.27\\
0.00603254823975779	0.27\\
0.00603254823975779	0.28\\
0.00612865636514691	0.28\\
0.00612865636514691	0.29\\
0.0061630099478404	0.29\\
0.0061630099478404	0.3\\
0.00617432934146672	0.3\\
0.00617432934146672	0.31\\
0.00618994226040939	0.31\\
0.00618994226040939	0.32\\
0.00620976839154533	0.32\\
0.00620976839154533	0.33\\
0.00621589041047224	0.33\\
0.00621589041047224	0.34\\
0.00622299644651732	0.34\\
0.00622299644651732	0.35\\
0.0062343259165862	0.35\\
0.0062343259165862	0.36\\
0.00627648039045602	0.36\\
0.00627648039045602	0.37\\
0.00634545501416627	0.37\\
0.00634545501416627	0.38\\
0.00637730768160198	0.38\\
0.00637730768160198	0.39\\
0.00640788564009761	0.39\\
0.00640788564009761	0.4\\
0.006415855404117	0.4\\
0.006415855404117	0.41\\
0.00646372169868585	0.41\\
0.00646372169868585	0.42\\
0.00654699862180399	0.42\\
0.00654699862180399	0.43\\
0.00656728063394036	0.43\\
0.00656728063394036	0.44\\
0.00658800268562385	0.44\\
0.00658800268562385	0.45\\
0.00661947482080476	0.45\\
0.00661947482080476	0.46\\
0.00671287872309909	0.46\\
0.00671287872309909	0.47\\
0.00673209634434497	0.47\\
0.00673209634434497	0.48\\
0.00673873996814358	0.48\\
0.00673873996814358	0.49\\
0.00676493352657311	0.49\\
0.00676493352657311	0.5\\
0.00678293182547686	0.5\\
0.00678293182547686	0.51\\
0.0067864636826908	0.51\\
0.0067864636826908	0.52\\
0.00688843352181448	0.52\\
0.00688843352181448	0.53\\
0.00690218623404389	0.53\\
0.00690218623404389	0.54\\
0.00692059412019435	0.54\\
0.00692059412019435	0.55\\
0.00695228513937172	0.55\\
0.00695228513937172	0.56\\
0.00696268765805748	0.56\\
0.00696268765805748	0.57\\
0.00698901995086007	0.57\\
0.00698901995086007	0.58\\
0.00701887482569471	0.58\\
0.00701887482569471	0.59\\
0.0070881888437203	0.59\\
0.0070881888437203	0.6\\
0.00709133457158546	0.6\\
0.00709133457158546	0.61\\
0.00709938665983232	0.61\\
0.00709938665983232	0.62\\
0.0071103192620758	0.62\\
0.0071103192620758	0.63\\
0.00714802314516168	0.63\\
0.00714802314516168	0.64\\
0.00717948379555864	0.64\\
0.00717948379555864	0.65\\
0.00720661799340744	0.65\\
0.00720661799340744	0.66\\
0.00721072490628053	0.66\\
0.00721072490628053	0.67\\
0.00727713275796887	0.67\\
0.00727713275796887	0.68\\
0.00733014380839564	0.68\\
0.00733014380839564	0.69\\
0.00734040335966124	0.69\\
0.00734040335966124	0.7\\
0.00736378800319066	0.7\\
0.00736378800319066	0.71\\
0.00736572374519651	0.71\\
0.00736572374519651	0.72\\
0.0073765123257748	0.72\\
0.0073765123257748	0.73\\
0.00741673477843082	0.73\\
0.00741673477843082	0.74\\
0.00749952340862622	0.74\\
0.00749952340862622	0.75\\
0.00753265357893415	0.75\\
0.00753265357893415	0.76\\
0.00754037977442961	0.76\\
0.00754037977442961	0.77\\
0.00758943452362781	0.77\\
0.00758943452362781	0.78\\
0.00761475721000997	0.78\\
0.00761475721000997	0.79\\
0.0077412746042716	0.79\\
0.0077412746042716	0.8\\
0.00776843123485257	0.8\\
0.00776843123485257	0.81\\
0.00783275913583604	0.81\\
0.00783275913583604	0.82\\
0.00791905001768998	0.82\\
0.00791905001768998	0.83\\
0.00807806751081398	0.83\\
0.00807806751081398	0.84\\
0.00813986797387923	0.84\\
0.00813986797387923	0.85\\
0.00825723615635137	0.85\\
0.00825723615635137	0.86\\
0.0082713869507189	0.86\\
0.0082713869507189	0.87\\
0.00831161454742953	0.87\\
0.00831161454742953	0.88\\
0.00851917175990109	0.88\\
0.00851917175990109	0.89\\
0.0085322476072092	0.89\\
0.0085322476072092	0.9\\
0.00861277743903294	0.9\\
0.00861277743903294	0.91\\
0.00865109615772425	0.91\\
0.00865109615772425	0.92\\
0.00872005431699495	0.92\\
0.00872005431699495	0.93\\
0.00872265152206257	0.93\\
0.00872265152206257	0.94\\
0.00880711469000858	0.94\\
0.00880711469000858	0.95\\
0.00888147476122421	0.95\\
0.00888147476122421	0.96\\
0.00943840673278368	0.96\\
0.00943840673278368	0.97\\
0.00945555000782478	0.97\\
0.00945555000782478	0.98\\
0.00978202883359448	0.98\\
0.00978202883359448	0.99\\
0.00994107140898879	0.99\\
0.00994107140898879	1\\
inf	1\\
};
\addplot [color=mycolor1, forget plot,line width=1.5]
  table[row sep=crcr]{%
-inf	0\\
0.00594100985237028	0\\
0.00594100985237028	0.01\\
0.00599009318527625	0.01\\
0.00599009318527625	0.02\\
0.00608293910923256	0.02\\
0.00608293910923256	0.03\\
0.00612100166685542	0.03\\
0.00612100166685542	0.04\\
0.0061438320642927	0.04\\
0.0061438320642927	0.05\\
0.00619205557790499	0.05\\
0.00619205557790499	0.06\\
0.00620959461818174	0.06\\
0.00620959461818174	0.07\\
0.00626229810250843	0.07\\
0.00626229810250843	0.08\\
0.00628484051723775	0.08\\
0.00628484051723775	0.09\\
0.00628787260249079	0.09\\
0.00628787260249079	0.1\\
0.00630051532259005	0.1\\
0.00630051532259005	0.11\\
0.00630513895786879	0.11\\
0.00630513895786879	0.12\\
0.00639814449263139	0.12\\
0.00639814449263139	0.13\\
0.00639999018185661	0.13\\
0.00639999018185661	0.14\\
0.00642100695036684	0.14\\
0.00642100695036684	0.15\\
0.0064223267240867	0.15\\
0.0064223267240867	0.16\\
0.00644484772732915	0.16\\
0.00644484772732915	0.17\\
0.00648379520670121	0.17\\
0.00648379520670121	0.18\\
0.00648595849995988	0.18\\
0.00648595849995988	0.19\\
0.0065160669128008	0.19\\
0.0065160669128008	0.2\\
0.00651800783203751	0.2\\
0.00651800783203751	0.21\\
0.00653780348947287	0.21\\
0.00653780348947287	0.22\\
0.00655071835161352	0.22\\
0.00655071835161352	0.23\\
0.00655097699606874	0.23\\
0.00655097699606874	0.24\\
0.00656035999919366	0.24\\
0.00656035999919366	0.25\\
0.00656521033430283	0.25\\
0.00656521033430283	0.26\\
0.00656770409220368	0.26\\
0.00656770409220368	0.27\\
0.00657314285487407	0.27\\
0.00657314285487407	0.28\\
0.00660724824334752	0.28\\
0.00660724824334752	0.29\\
0.00661443603215063	0.29\\
0.00661443603215063	0.3\\
0.00661949165534638	0.3\\
0.00661949165534638	0.31\\
0.00662172939798818	0.31\\
0.00662172939798818	0.32\\
0.0066234818202168	0.32\\
0.0066234818202168	0.33\\
0.00663655304330502	0.33\\
0.00663655304330502	0.34\\
0.00666537258185465	0.34\\
0.00666537258185465	0.35\\
0.00666997356377142	0.35\\
0.00666997356377142	0.36\\
0.00668990634013947	0.36\\
0.00668990634013947	0.37\\
0.00669850296160555	0.37\\
0.00669850296160555	0.38\\
0.00672666207867346	0.38\\
0.00672666207867346	0.39\\
0.00672793821785664	0.39\\
0.00672793821785664	0.4\\
0.00673900999319645	0.4\\
0.00673900999319645	0.41\\
0.0067480603076519	0.41\\
0.0067480603076519	0.42\\
0.00679255448276614	0.42\\
0.00679255448276614	0.43\\
0.00680142826592546	0.43\\
0.00680142826592546	0.44\\
0.00680652403559258	0.44\\
0.00680652403559258	0.45\\
0.0068112915584925	0.45\\
0.0068112915584925	0.46\\
0.0068114050883781	0.46\\
0.0068114050883781	0.47\\
0.00681325895554897	0.47\\
0.00681325895554897	0.48\\
0.00682774836370451	0.48\\
0.00682774836370451	0.49\\
0.00682867776816079	0.49\\
0.00682867776816079	0.5\\
0.00686081372727172	0.5\\
0.00686081372727172	0.51\\
0.00687319130309085	0.51\\
0.00687319130309085	0.52\\
0.00687560549718734	0.52\\
0.00687560549718734	0.53\\
0.00688041209843295	0.53\\
0.00688041209843295	0.54\\
0.00688322308744301	0.54\\
0.00688322308744301	0.55\\
0.00689341480763436	0.55\\
0.00689341480763436	0.56\\
0.00690180459866101	0.56\\
0.00690180459866101	0.57\\
0.00690631648921724	0.57\\
0.00690631648921724	0.58\\
0.00692350250255314	0.58\\
0.00692350250255314	0.59\\
0.00692415714623772	0.59\\
0.00692415714623772	0.6\\
0.00692706459492213	0.6\\
0.00692706459492213	0.61\\
0.00692811521293472	0.61\\
0.00692811521293472	0.62\\
0.00694132508060988	0.62\\
0.00694132508060988	0.63\\
0.00694747027538867	0.63\\
0.00694747027538867	0.64\\
0.00696447902670257	0.64\\
0.00696447902670257	0.65\\
0.00697885218236809	0.65\\
0.00697885218236809	0.66\\
0.00697998994538625	0.66\\
0.00697998994538625	0.67\\
0.00698089026183617	0.67\\
0.00698089026183617	0.68\\
0.00698886050575452	0.68\\
0.00698886050575452	0.69\\
0.00699347728704452	0.69\\
0.00699347728704452	0.7\\
0.00699445228160716	0.7\\
0.00699445228160716	0.71\\
0.00700024363357147	0.71\\
0.00700024363357147	0.72\\
0.00703515647796582	0.72\\
0.00703515647796582	0.73\\
0.00705293919011259	0.73\\
0.00705293919011259	0.74\\
0.00706666840442122	0.74\\
0.00706666840442122	0.75\\
0.00707374338173634	0.75\\
0.00707374338173634	0.76\\
0.00707935883172926	0.76\\
0.00707935883172926	0.77\\
0.00708973165635371	0.77\\
0.00708973165635371	0.78\\
0.00709033204312792	0.78\\
0.00709033204312792	0.79\\
0.00712502611020385	0.79\\
0.00712502611020385	0.8\\
0.00714302264006296	0.8\\
0.00714302264006296	0.81\\
0.00715106481882321	0.81\\
0.00715106481882321	0.82\\
0.00715558175162197	0.82\\
0.00715558175162197	0.83\\
0.00716296788994827	0.83\\
0.00716296788994827	0.84\\
0.0071717992877789	0.84\\
0.0071717992877789	0.85\\
0.00719582884520419	0.85\\
0.00719582884520419	0.86\\
0.00719978994612414	0.86\\
0.00719978994612414	0.87\\
0.00725214656916683	0.87\\
0.00725214656916683	0.88\\
0.0072559042471206	0.88\\
0.0072559042471206	0.89\\
0.00727206028014622	0.89\\
0.00727206028014622	0.9\\
0.0073002894567794	0.9\\
0.0073002894567794	0.91\\
0.00730865983457664	0.91\\
0.00730865983457664	0.92\\
0.00732552008791973	0.92\\
0.00732552008791973	0.93\\
0.00740587093370403	0.93\\
0.00740587093370403	0.94\\
0.00743721550781977	0.94\\
0.00743721550781977	0.95\\
0.00754312957575401	0.95\\
0.00754312957575401	0.96\\
0.00760432749786826	0.96\\
0.00760432749786826	0.97\\
0.00766434998081241	0.97\\
0.00766434998081241	0.98\\
0.00768174563188015	0.98\\
0.00768174563188015	0.99\\
0.00778197997001614	0.99\\
0.00778197997001614	1\\
inf	1\\
};
\draw (axis cs:.007,.6) ellipse (.2cm and .1cm);
\draw (axis cs:.0002,.5) ellipse (.2cm and .1cm);
\addplot [color=mycolor2, forget plot,line width=1.5,dashed]
  table[row sep=crcr]{%
-inf	0\\
0.00388763495332524	0\\
0.00388763495332524	0.01\\
0.0039779769369078	0.01\\
0.0039779769369078	0.02\\
0.00437702219895772	0.02\\
0.00437702219895772	0.03\\
0.0045279377194668	0.03\\
0.0045279377194668	0.04\\
0.00456982329175554	0.04\\
0.00456982329175554	0.05\\
0.00483098405479953	0.05\\
0.00483098405479953	0.06\\
0.00494256970577131	0.06\\
0.00494256970577131	0.07\\
0.00501030301268805	0.07\\
0.00501030301268805	0.08\\
0.00513783394341532	0.08\\
0.00513783394341532	0.09\\
0.00519586445469606	0.09\\
0.00519586445469606	0.1\\
0.00523357784167244	0.1\\
0.00523357784167244	0.11\\
0.00525944393745265	0.11\\
0.00525944393745265	0.12\\
0.00531603796773738	0.12\\
0.00531603796773738	0.13\\
0.00541826257025269	0.13\\
0.00541826257025269	0.14\\
0.00543579830221148	0.14\\
0.00543579830221148	0.15\\
0.00547540416269369	0.15\\
0.00547540416269369	0.16\\
0.0054851530725855	0.16\\
0.0054851530725855	0.17\\
0.00550140659815427	0.17\\
0.00550140659815427	0.18\\
0.00552060998763975	0.18\\
0.00552060998763975	0.19\\
0.00555979050277402	0.19\\
0.00555979050277402	0.2\\
0.00556285059006915	0.2\\
0.00556285059006915	0.21\\
0.00568453435581969	0.21\\
0.00568453435581969	0.22\\
0.00569204200507351	0.22\\
0.00569204200507351	0.23\\
0.00579280694758293	0.23\\
0.00579280694758293	0.24\\
0.00579995431037703	0.24\\
0.00579995431037703	0.25\\
0.00588773873775303	0.25\\
0.00588773873775303	0.26\\
0.00593842205392088	0.26\\
0.00593842205392088	0.27\\
0.00603254823975779	0.27\\
0.00603254823975779	0.28\\
0.00612865636514691	0.28\\
0.00612865636514691	0.29\\
0.0061630099478404	0.29\\
0.0061630099478404	0.3\\
0.00617432934146672	0.3\\
0.00617432934146672	0.31\\
0.00618994226040939	0.31\\
0.00618994226040939	0.32\\
0.00620976839154533	0.32\\
0.00620976839154533	0.33\\
0.00621589041047224	0.33\\
0.00621589041047224	0.34\\
0.00622299644651732	0.34\\
0.00622299644651732	0.35\\
0.0062343259165862	0.35\\
0.0062343259165862	0.36\\
0.00627648039045602	0.36\\
0.00627648039045602	0.37\\
0.00634545501416627	0.37\\
0.00634545501416627	0.38\\
0.00637730768160198	0.38\\
0.00637730768160198	0.39\\
0.00640788564009761	0.39\\
0.00640788564009761	0.4\\
0.006415855404117	0.4\\
0.006415855404117	0.41\\
0.00646372169868585	0.41\\
0.00646372169868585	0.42\\
0.00654699862180399	0.42\\
0.00654699862180399	0.43\\
0.00656728063394036	0.43\\
0.00656728063394036	0.44\\
0.00658800268562385	0.44\\
0.00658800268562385	0.45\\
0.00661947482080476	0.45\\
0.00661947482080476	0.46\\
0.00671287872309909	0.46\\
0.00671287872309909	0.47\\
0.00673209634434497	0.47\\
0.00673209634434497	0.48\\
0.00673873996814358	0.48\\
0.00673873996814358	0.49\\
0.00676493352657311	0.49\\
0.00676493352657311	0.5\\
0.00678293182547686	0.5\\
0.00678293182547686	0.51\\
0.0067864636826908	0.51\\
0.0067864636826908	0.52\\
0.00688843352181448	0.52\\
0.00688843352181448	0.53\\
0.00690218623404389	0.53\\
0.00690218623404389	0.54\\
0.00692059412019435	0.54\\
0.00692059412019435	0.55\\
0.00695228513937172	0.55\\
0.00695228513937172	0.56\\
0.00696268765805748	0.56\\
0.00696268765805748	0.57\\
0.00698901995086007	0.57\\
0.00698901995086007	0.58\\
0.00701887482569471	0.58\\
0.00701887482569471	0.59\\
0.0070881888437203	0.59\\
0.0070881888437203	0.6\\
0.00709133457158546	0.6\\
0.00709133457158546	0.61\\
0.00709938665983232	0.61\\
0.00709938665983232	0.62\\
0.0071103192620758	0.62\\
0.0071103192620758	0.63\\
0.00714802314516168	0.63\\
0.00714802314516168	0.64\\
0.00717948379555864	0.64\\
0.00717948379555864	0.65\\
0.00720661799340744	0.65\\
0.00720661799340744	0.66\\
0.00721072490628053	0.66\\
0.00721072490628053	0.67\\
0.00727713275796887	0.67\\
0.00727713275796887	0.68\\
0.00733014380839564	0.68\\
0.00733014380839564	0.69\\
0.00734040335966124	0.69\\
0.00734040335966124	0.7\\
0.00736378800319066	0.7\\
0.00736378800319066	0.71\\
0.00736572374519651	0.71\\
0.00736572374519651	0.72\\
0.0073765123257748	0.72\\
0.0073765123257748	0.73\\
0.00741673477843082	0.73\\
0.00741673477843082	0.74\\
0.00749952340862622	0.74\\
0.00749952340862622	0.75\\
0.00753265357893415	0.75\\
0.00753265357893415	0.76\\
0.00754037977442961	0.76\\
0.00754037977442961	0.77\\
0.00758943452362781	0.77\\
0.00758943452362781	0.78\\
0.00761475721000997	0.78\\
0.00761475721000997	0.79\\
0.0077412746042716	0.79\\
0.0077412746042716	0.8\\
0.00776843123485257	0.8\\
0.00776843123485257	0.81\\
0.00783275913583604	0.81\\
0.00783275913583604	0.82\\
0.00791905001768998	0.82\\
0.00791905001768998	0.83\\
0.00807806751081398	0.83\\
0.00807806751081398	0.84\\
0.00813986797387923	0.84\\
0.00813986797387923	0.85\\
0.00825723615635137	0.85\\
0.00825723615635137	0.86\\
0.0082713869507189	0.86\\
0.0082713869507189	0.87\\
0.00831161454742953	0.87\\
0.00831161454742953	0.88\\
0.00851917175990109	0.88\\
0.00851917175990109	0.89\\
0.0085322476072092	0.89\\
0.0085322476072092	0.9\\
0.00861277743903294	0.9\\
0.00861277743903294	0.91\\
0.00865109615772425	0.91\\
0.00865109615772425	0.92\\
0.00872005431699495	0.92\\
0.00872005431699495	0.93\\
0.00872265152206257	0.93\\
0.00872265152206257	0.94\\
0.00880711469000858	0.94\\
0.00880711469000858	0.95\\
0.00888147476122421	0.95\\
0.00888147476122421	0.96\\
0.00943840673278368	0.96\\
0.00943840673278368	0.97\\
0.00945555000782478	0.97\\
0.00945555000782478	0.98\\
0.00978202883359448	0.98\\
0.00978202883359448	0.99\\
0.00994107140898879	0.99\\
0.00994107140898879	1\\
inf	1\\
};
\addplot [color=mycolor1, forget plot,line width=1.5]
  table[row sep=crcr]{%
-inf	0\\
0.00594100985237028	0\\
0.00594100985237028	0.01\\
0.00599009318527625	0.01\\
0.00599009318527625	0.02\\
0.00608293910923256	0.02\\
0.00608293910923256	0.03\\
0.00612100166685542	0.03\\
0.00612100166685542	0.04\\
0.0061438320642927	0.04\\
0.0061438320642927	0.05\\
0.00619205557790499	0.05\\
0.00619205557790499	0.06\\
0.00620959461818174	0.06\\
0.00620959461818174	0.07\\
0.00626229810250843	0.07\\
0.00626229810250843	0.08\\
0.00628484051723775	0.08\\
0.00628484051723775	0.09\\
0.00628787260249079	0.09\\
0.00628787260249079	0.1\\
0.00630051532259005	0.1\\
0.00630051532259005	0.11\\
0.00630513895786879	0.11\\
0.00630513895786879	0.12\\
0.00639814449263139	0.12\\
0.00639814449263139	0.13\\
0.00639999018185661	0.13\\
0.00639999018185661	0.14\\
0.00642100695036684	0.14\\
0.00642100695036684	0.15\\
0.0064223267240867	0.15\\
0.0064223267240867	0.16\\
0.00644484772732915	0.16\\
0.00644484772732915	0.17\\
0.00648379520670121	0.17\\
0.00648379520670121	0.18\\
0.00648595849995988	0.18\\
0.00648595849995988	0.19\\
0.0065160669128008	0.19\\
0.0065160669128008	0.2\\
0.00651800783203751	0.2\\
0.00651800783203751	0.21\\
0.00653780348947287	0.21\\
0.00653780348947287	0.22\\
0.00655071835161352	0.22\\
0.00655071835161352	0.23\\
0.00655097699606874	0.23\\
0.00655097699606874	0.24\\
0.00656035999919366	0.24\\
0.00656035999919366	0.25\\
0.00656521033430283	0.25\\
0.00656521033430283	0.26\\
0.00656770409220368	0.26\\
0.00656770409220368	0.27\\
0.00657314285487407	0.27\\
0.00657314285487407	0.28\\
0.00660724824334752	0.28\\
0.00660724824334752	0.29\\
0.00661443603215063	0.29\\
0.00661443603215063	0.3\\
0.00661949165534638	0.3\\
0.00661949165534638	0.31\\
0.00662172939798818	0.31\\
0.00662172939798818	0.32\\
0.0066234818202168	0.32\\
0.0066234818202168	0.33\\
0.00663655304330502	0.33\\
0.00663655304330502	0.34\\
0.00666537258185465	0.34\\
0.00666537258185465	0.35\\
0.00666997356377142	0.35\\
0.00666997356377142	0.36\\
0.00668990634013947	0.36\\
0.00668990634013947	0.37\\
0.00669850296160555	0.37\\
0.00669850296160555	0.38\\
0.00672666207867346	0.38\\
0.00672666207867346	0.39\\
0.00672793821785664	0.39\\
0.00672793821785664	0.4\\
0.00673900999319645	0.4\\
0.00673900999319645	0.41\\
0.0067480603076519	0.41\\
0.0067480603076519	0.42\\
0.00679255448276614	0.42\\
0.00679255448276614	0.43\\
0.00680142826592546	0.43\\
0.00680142826592546	0.44\\
0.00680652403559258	0.44\\
0.00680652403559258	0.45\\
0.0068112915584925	0.45\\
0.0068112915584925	0.46\\
0.0068114050883781	0.46\\
0.0068114050883781	0.47\\
0.00681325895554897	0.47\\
0.00681325895554897	0.48\\
0.00682774836370451	0.48\\
0.00682774836370451	0.49\\
0.00682867776816079	0.49\\
0.00682867776816079	0.5\\
0.00686081372727172	0.5\\
0.00686081372727172	0.51\\
0.00687319130309085	0.51\\
0.00687319130309085	0.52\\
0.00687560549718734	0.52\\
0.00687560549718734	0.53\\
0.00688041209843295	0.53\\
0.00688041209843295	0.54\\
0.00688322308744301	0.54\\
0.00688322308744301	0.55\\
0.00689341480763436	0.55\\
0.00689341480763436	0.56\\
0.00690180459866101	0.56\\
0.00690180459866101	0.57\\
0.00690631648921724	0.57\\
0.00690631648921724	0.58\\
0.00692350250255314	0.58\\
0.00692350250255314	0.59\\
0.00692415714623772	0.59\\
0.00692415714623772	0.6\\
0.00692706459492213	0.6\\
0.00692706459492213	0.61\\
0.00692811521293472	0.61\\
0.00692811521293472	0.62\\
0.00694132508060988	0.62\\
0.00694132508060988	0.63\\
0.00694747027538867	0.63\\
0.00694747027538867	0.64\\
0.00696447902670257	0.64\\
0.00696447902670257	0.65\\
0.00697885218236809	0.65\\
0.00697885218236809	0.66\\
0.00697998994538625	0.66\\
0.00697998994538625	0.67\\
0.00698089026183617	0.67\\
0.00698089026183617	0.68\\
0.00698886050575452	0.68\\
0.00698886050575452	0.69\\
0.00699347728704452	0.69\\
0.00699347728704452	0.7\\
0.00699445228160716	0.7\\
0.00699445228160716	0.71\\
0.00700024363357147	0.71\\
0.00700024363357147	0.72\\
0.00703515647796582	0.72\\
0.00703515647796582	0.73\\
0.00705293919011259	0.73\\
0.00705293919011259	0.74\\
0.00706666840442122	0.74\\
0.00706666840442122	0.75\\
0.00707374338173634	0.75\\
0.00707374338173634	0.76\\
0.00707935883172926	0.76\\
0.00707935883172926	0.77\\
0.00708973165635371	0.77\\
0.00708973165635371	0.78\\
0.00709033204312792	0.78\\
0.00709033204312792	0.79\\
0.00712502611020385	0.79\\
0.00712502611020385	0.8\\
0.00714302264006296	0.8\\
0.00714302264006296	0.81\\
0.00715106481882321	0.81\\
0.00715106481882321	0.82\\
0.00715558175162197	0.82\\
0.00715558175162197	0.83\\
0.00716296788994827	0.83\\
0.00716296788994827	0.84\\
0.0071717992877789	0.84\\
0.0071717992877789	0.85\\
0.00719582884520419	0.85\\
0.00719582884520419	0.86\\
0.00719978994612414	0.86\\
0.00719978994612414	0.87\\
0.00725214656916683	0.87\\
0.00725214656916683	0.88\\
0.0072559042471206	0.88\\
0.0072559042471206	0.89\\
0.00727206028014622	0.89\\
0.00727206028014622	0.9\\
0.0073002894567794	0.9\\
0.0073002894567794	0.91\\
0.00730865983457664	0.91\\
0.00730865983457664	0.92\\
0.00732552008791973	0.92\\
0.00732552008791973	0.93\\
0.00740587093370403	0.93\\
0.00740587093370403	0.94\\
0.00743721550781977	0.94\\
0.00743721550781977	0.95\\
0.00754312957575401	0.95\\
0.00754312957575401	0.96\\
0.00760432749786826	0.96\\
0.00760432749786826	0.97\\
0.00766434998081241	0.97\\
0.00766434998081241	0.98\\
0.00768174563188015	0.98\\
0.00768174563188015	0.99\\
0.00778197997001614	0.99\\
0.00778197997001614	1\\
inf	1\\
};
\addplot [color=mycolor4, forget plot,line width=1.5,dashed]
  table[row sep=crcr]{%
-inf	0\\
0.00011232224903237	0\\
0.00011232224903237	0.01\\
0.000132664259120409	0.01\\
0.000132664259120409	0.02\\
0.000135440705014567	0.02\\
0.000135440705014567	0.03\\
0.000137999779111252	0.03\\
0.000137999779111252	0.04\\
0.000139777631935138	0.04\\
0.000139777631935138	0.05\\
0.000144798553852591	0.05\\
0.000144798553852591	0.06\\
0.0001454215399217	0.06\\
0.0001454215399217	0.07\\
0.000146148071813339	0.07\\
0.000146148071813339	0.08\\
0.000151615712039857	0.08\\
0.000151615712039857	0.09\\
0.000152188939301633	0.09\\
0.000152188939301633	0.1\\
0.000153389718098912	0.1\\
0.000153389718098912	0.11\\
0.000155881877449653	0.11\\
0.000155881877449653	0.12\\
0.000159475196603521	0.12\\
0.000159475196603521	0.13\\
0.000162393021939165	0.13\\
0.000162393021939165	0.14\\
0.000162481736185424	0.14\\
0.000162481736185424	0.15\\
0.00016355839167028	0.15\\
0.00016355839167028	0.16\\
0.000164360212165144	0.16\\
0.000164360212165144	0.17\\
0.000166205628664413	0.17\\
0.000166205628664413	0.18\\
0.00016729967128035	0.18\\
0.00016729967128035	0.19\\
0.000167543972248635	0.19\\
0.000167543972248635	0.2\\
0.000168199159672017	0.2\\
0.000168199159672017	0.21\\
0.000168753160316601	0.21\\
0.000168753160316601	0.22\\
0.000170104066424328	0.22\\
0.000170104066424328	0.23\\
0.000171998178883475	0.23\\
0.000171998178883475	0.24\\
0.000172393757545375	0.24\\
0.000172393757545375	0.25\\
0.000172838328136889	0.25\\
0.000172838328136889	0.26\\
0.000173113337119311	0.26\\
0.000173113337119311	0.27\\
0.000173944450549086	0.27\\
0.000173944450549086	0.28\\
0.000175000527534652	0.28\\
0.000175000527534652	0.29\\
0.000175031242330986	0.29\\
0.000175031242330986	0.3\\
0.000175049882536907	0.3\\
0.000175049882536907	0.31\\
0.00017685385417011	0.31\\
0.00017685385417011	0.32\\
0.00017721340298952	0.32\\
0.00017721340298952	0.33\\
0.000178382725188189	0.33\\
0.000178382725188189	0.34\\
0.000179968888655554	0.34\\
0.000179968888655554	0.35\\
0.000180381275025027	0.35\\
0.000180381275025027	0.36\\
0.000182263019250601	0.36\\
0.000182263019250601	0.37\\
0.000184351631466098	0.37\\
0.000184351631466098	0.38\\
0.000185690609388068	0.38\\
0.000185690609388068	0.39\\
0.000185809971110344	0.39\\
0.000185809971110344	0.4\\
0.000186484144343535	0.4\\
0.000186484144343535	0.41\\
0.000186727973380558	0.41\\
0.000186727973380558	0.42\\
0.000187789617452051	0.42\\
0.000187789617452051	0.43\\
0.000190878716688063	0.43\\
0.000190878716688063	0.44\\
0.000192092391078644	0.44\\
0.000192092391078644	0.45\\
0.0001925708057419	0.45\\
0.0001925708057419	0.46\\
0.000192825329902341	0.46\\
0.000192825329902341	0.47\\
0.00019574668049318	0.47\\
0.00019574668049318	0.48\\
0.000196054427259001	0.48\\
0.000196054427259001	0.49\\
0.000196066120994377	0.49\\
0.000196066120994377	0.5\\
0.000196243712916713	0.5\\
0.000196243712916713	0.51\\
0.000197908542453539	0.51\\
0.000197908542453539	0.52\\
0.000199951866781676	0.52\\
0.000199951866781676	0.53\\
0.000201967012243252	0.53\\
0.000201967012243252	0.54\\
0.000204583495005922	0.54\\
0.000204583495005922	0.55\\
0.000205083620511362	0.55\\
0.000205083620511362	0.56\\
0.000206217822033662	0.56\\
0.000206217822033662	0.57\\
0.000210588176358721	0.57\\
0.000210588176358721	0.58\\
0.000210891628503493	0.58\\
0.000210891628503493	0.59\\
0.000211612889490476	0.59\\
0.000211612889490476	0.6\\
0.000216704452699321	0.6\\
0.000216704452699321	0.61\\
0.00021792486168125	0.61\\
0.00021792486168125	0.62\\
0.00021880506567007	0.62\\
0.00021880506567007	0.63\\
0.000220244805660615	0.63\\
0.000220244805660615	0.64\\
0.000223864472688557	0.64\\
0.000223864472688557	0.65\\
0.000225482117588474	0.65\\
0.000225482117588474	0.66\\
0.000235902796234541	0.66\\
0.000235902796234541	0.67\\
0.000236873568457471	0.67\\
0.000236873568457471	0.68\\
0.000238717174074063	0.68\\
0.000238717174074063	0.69\\
0.000240600914805742	0.69\\
0.000240600914805742	0.7\\
0.000242010799241503	0.7\\
0.000242010799241503	0.71\\
0.000248589256914538	0.71\\
0.000248589256914538	0.72\\
0.000248853053106988	0.72\\
0.000248853053106988	0.73\\
0.000249579117032489	0.73\\
0.000249579117032489	0.74\\
0.00025030545113763	0.74\\
0.00025030545113763	0.75\\
0.000251515601330918	0.75\\
0.000251515601330918	0.76\\
0.000255359436627307	0.76\\
0.000255359436627307	0.77\\
0.000255591279058822	0.77\\
0.000255591279058822	0.78\\
0.000257462691045095	0.78\\
0.000257462691045095	0.79\\
0.000259044884009224	0.79\\
0.000259044884009224	0.8\\
0.000263163762063586	0.8\\
0.000263163762063586	0.81\\
0.000265082226469375	0.81\\
0.000265082226469375	0.82\\
0.000270683907654262	0.82\\
0.000270683907654262	0.83\\
0.000271794779947823	0.83\\
0.000271794779947823	0.84\\
0.000274334055882935	0.84\\
0.000274334055882935	0.85\\
0.000275601789897137	0.85\\
0.000275601789897137	0.86\\
0.00027659085624157	0.86\\
0.00027659085624157	0.87\\
0.000276598188193763	0.87\\
0.000276598188193763	0.88\\
0.000279274580375057	0.88\\
0.000279274580375057	0.89\\
0.000284652041007721	0.89\\
0.000284652041007721	0.9\\
0.000289244724459333	0.9\\
0.000289244724459333	0.91\\
0.000294055228010513	0.91\\
0.000294055228010513	0.92\\
0.000295103004695487	0.92\\
0.000295103004695487	0.93\\
0.000301143470761249	0.93\\
0.000301143470761249	0.94\\
0.000306698642341025	0.94\\
0.000306698642341025	0.95\\
0.000309825544728867	0.95\\
0.000309825544728867	0.96\\
0.000312107851901522	0.96\\
0.000312107851901522	0.97\\
0.000317339375649714	0.97\\
0.000317339375649714	0.98\\
0.000352791213145002	0.98\\
0.000352791213145002	0.99\\
0.295800980029507	0.99\\
0.295800980029507	1\\
inf	1\\
};
\addplot [color=mycolor1, forget plot,line width=1.5]
  table[row sep=crcr]{%
-inf	0\\
0.00594100985237028	0\\
0.00594100985237028	0.01\\
0.00599009318527625	0.01\\
0.00599009318527625	0.02\\
0.00608293910923256	0.02\\
0.00608293910923256	0.03\\
0.00612100166685542	0.03\\
0.00612100166685542	0.04\\
0.0061438320642927	0.04\\
0.0061438320642927	0.05\\
0.00619205557790499	0.05\\
0.00619205557790499	0.06\\
0.00620959461818174	0.06\\
0.00620959461818174	0.07\\
0.00626229810250843	0.07\\
0.00626229810250843	0.08\\
0.00628484051723775	0.08\\
0.00628484051723775	0.09\\
0.00628787260249079	0.09\\
0.00628787260249079	0.1\\
0.00630051532259005	0.1\\
0.00630051532259005	0.11\\
0.00630513895786879	0.11\\
0.00630513895786879	0.12\\
0.00639814449263139	0.12\\
0.00639814449263139	0.13\\
0.00639999018185661	0.13\\
0.00639999018185661	0.14\\
0.00642100695036684	0.14\\
0.00642100695036684	0.15\\
0.0064223267240867	0.15\\
0.0064223267240867	0.16\\
0.00644484772732915	0.16\\
0.00644484772732915	0.17\\
0.00648379520670121	0.17\\
0.00648379520670121	0.18\\
0.00648595849995988	0.18\\
0.00648595849995988	0.19\\
0.0065160669128008	0.19\\
0.0065160669128008	0.2\\
0.00651800783203751	0.2\\
0.00651800783203751	0.21\\
0.00653780348947287	0.21\\
0.00653780348947287	0.22\\
0.00655071835161352	0.22\\
0.00655071835161352	0.23\\
0.00655097699606874	0.23\\
0.00655097699606874	0.24\\
0.00656035999919366	0.24\\
0.00656035999919366	0.25\\
0.00656521033430283	0.25\\
0.00656521033430283	0.26\\
0.00656770409220368	0.26\\
0.00656770409220368	0.27\\
0.00657314285487407	0.27\\
0.00657314285487407	0.28\\
0.00660724824334752	0.28\\
0.00660724824334752	0.29\\
0.00661443603215063	0.29\\
0.00661443603215063	0.3\\
0.00661949165534638	0.3\\
0.00661949165534638	0.31\\
0.00662172939798818	0.31\\
0.00662172939798818	0.32\\
0.0066234818202168	0.32\\
0.0066234818202168	0.33\\
0.00663655304330502	0.33\\
0.00663655304330502	0.34\\
0.00666537258185465	0.34\\
0.00666537258185465	0.35\\
0.00666997356377142	0.35\\
0.00666997356377142	0.36\\
0.00668990634013947	0.36\\
0.00668990634013947	0.37\\
0.00669850296160555	0.37\\
0.00669850296160555	0.38\\
0.00672666207867346	0.38\\
0.00672666207867346	0.39\\
0.00672793821785664	0.39\\
0.00672793821785664	0.4\\
0.00673900999319645	0.4\\
0.00673900999319645	0.41\\
0.0067480603076519	0.41\\
0.0067480603076519	0.42\\
0.00679255448276614	0.42\\
0.00679255448276614	0.43\\
0.00680142826592546	0.43\\
0.00680142826592546	0.44\\
0.00680652403559258	0.44\\
0.00680652403559258	0.45\\
0.0068112915584925	0.45\\
0.0068112915584925	0.46\\
0.0068114050883781	0.46\\
0.0068114050883781	0.47\\
0.00681325895554897	0.47\\
0.00681325895554897	0.48\\
0.00682774836370451	0.48\\
0.00682774836370451	0.49\\
0.00682867776816079	0.49\\
0.00682867776816079	0.5\\
0.00686081372727172	0.5\\
0.00686081372727172	0.51\\
0.00687319130309085	0.51\\
0.00687319130309085	0.52\\
0.00687560549718734	0.52\\
0.00687560549718734	0.53\\
0.00688041209843295	0.53\\
0.00688041209843295	0.54\\
0.00688322308744301	0.54\\
0.00688322308744301	0.55\\
0.00689341480763436	0.55\\
0.00689341480763436	0.56\\
0.00690180459866101	0.56\\
0.00690180459866101	0.57\\
0.00690631648921724	0.57\\
0.00690631648921724	0.58\\
0.00692350250255314	0.58\\
0.00692350250255314	0.59\\
0.00692415714623772	0.59\\
0.00692415714623772	0.6\\
0.00692706459492213	0.6\\
0.00692706459492213	0.61\\
0.00692811521293472	0.61\\
0.00692811521293472	0.62\\
0.00694132508060988	0.62\\
0.00694132508060988	0.63\\
0.00694747027538867	0.63\\
0.00694747027538867	0.64\\
0.00696447902670257	0.64\\
0.00696447902670257	0.65\\
0.00697885218236809	0.65\\
0.00697885218236809	0.66\\
0.00697998994538625	0.66\\
0.00697998994538625	0.67\\
0.00698089026183617	0.67\\
0.00698089026183617	0.68\\
0.00698886050575452	0.68\\
0.00698886050575452	0.69\\
0.00699347728704452	0.69\\
0.00699347728704452	0.7\\
0.00699445228160716	0.7\\
0.00699445228160716	0.71\\
0.00700024363357147	0.71\\
0.00700024363357147	0.72\\
0.00703515647796582	0.72\\
0.00703515647796582	0.73\\
0.00705293919011259	0.73\\
0.00705293919011259	0.74\\
0.00706666840442122	0.74\\
0.00706666840442122	0.75\\
0.00707374338173634	0.75\\
0.00707374338173634	0.76\\
0.00707935883172926	0.76\\
0.00707935883172926	0.77\\
0.00708973165635371	0.77\\
0.00708973165635371	0.78\\
0.00709033204312792	0.78\\
0.00709033204312792	0.79\\
0.00712502611020385	0.79\\
0.00712502611020385	0.8\\
0.00714302264006296	0.8\\
0.00714302264006296	0.81\\
0.00715106481882321	0.81\\
0.00715106481882321	0.82\\
0.00715558175162197	0.82\\
0.00715558175162197	0.83\\
0.00716296788994827	0.83\\
0.00716296788994827	0.84\\
0.0071717992877789	0.84\\
0.0071717992877789	0.85\\
0.00719582884520419	0.85\\
0.00719582884520419	0.86\\
0.00719978994612414	0.86\\
0.00719978994612414	0.87\\
0.00725214656916683	0.87\\
0.00725214656916683	0.88\\
0.0072559042471206	0.88\\
0.0072559042471206	0.89\\
0.00727206028014622	0.89\\
0.00727206028014622	0.9\\
0.0073002894567794	0.9\\
0.0073002894567794	0.91\\
0.00730865983457664	0.91\\
0.00730865983457664	0.92\\
0.00732552008791973	0.92\\
0.00732552008791973	0.93\\
0.00740587093370403	0.93\\
0.00740587093370403	0.94\\
0.00743721550781977	0.94\\
0.00743721550781977	0.95\\
0.00754312957575401	0.95\\
0.00754312957575401	0.96\\
0.00760432749786826	0.96\\
0.00760432749786826	0.97\\
0.00766434998081241	0.97\\
0.00766434998081241	0.98\\
0.00768174563188015	0.98\\
0.00768174563188015	0.99\\
0.00778197997001614	0.99\\
0.00778197997001614	1\\
inf	1\\
};
\addplot [color=mycolor4, forget plot,line width=1.5,dashed]
  table[row sep=crcr]{%
-inf	0\\
0.00011232224903237	0\\
0.00011232224903237	0.01\\
0.000132664259120409	0.01\\
0.000132664259120409	0.02\\
0.000135440705014567	0.02\\
0.000135440705014567	0.03\\
0.000137999779111252	0.03\\
0.000137999779111252	0.04\\
0.000139777631935138	0.04\\
0.000139777631935138	0.05\\
0.000144798553852591	0.05\\
0.000144798553852591	0.06\\
0.0001454215399217	0.06\\
0.0001454215399217	0.07\\
0.000146148071813339	0.07\\
0.000146148071813339	0.08\\
0.000151615712039857	0.08\\
0.000151615712039857	0.09\\
0.000152188939301633	0.09\\
0.000152188939301633	0.1\\
0.000153389718098912	0.1\\
0.000153389718098912	0.11\\
0.000155881877449653	0.11\\
0.000155881877449653	0.12\\
0.000159475196603521	0.12\\
0.000159475196603521	0.13\\
0.000162393021939165	0.13\\
0.000162393021939165	0.14\\
0.000162481736185424	0.14\\
0.000162481736185424	0.15\\
0.00016355839167028	0.15\\
0.00016355839167028	0.16\\
0.000164360212165144	0.16\\
0.000164360212165144	0.17\\
0.000166205628664413	0.17\\
0.000166205628664413	0.18\\
0.00016729967128035	0.18\\
0.00016729967128035	0.19\\
0.000167543972248635	0.19\\
0.000167543972248635	0.2\\
0.000168199159672017	0.2\\
0.000168199159672017	0.21\\
0.000168753160316601	0.21\\
0.000168753160316601	0.22\\
0.000170104066424328	0.22\\
0.000170104066424328	0.23\\
0.000171998178883475	0.23\\
0.000171998178883475	0.24\\
0.000172393757545375	0.24\\
0.000172393757545375	0.25\\
0.000172838328136889	0.25\\
0.000172838328136889	0.26\\
0.000173113337119311	0.26\\
0.000173113337119311	0.27\\
0.000173944450549086	0.27\\
0.000173944450549086	0.28\\
0.000175000527534652	0.28\\
0.000175000527534652	0.29\\
0.000175031242330986	0.29\\
0.000175031242330986	0.3\\
0.000175049882536907	0.3\\
0.000175049882536907	0.31\\
0.00017685385417011	0.31\\
0.00017685385417011	0.32\\
0.00017721340298952	0.32\\
0.00017721340298952	0.33\\
0.000178382725188189	0.33\\
0.000178382725188189	0.34\\
0.000179968888655554	0.34\\
0.000179968888655554	0.35\\
0.000180381275025027	0.35\\
0.000180381275025027	0.36\\
0.000182263019250601	0.36\\
0.000182263019250601	0.37\\
0.000184351631466098	0.37\\
0.000184351631466098	0.38\\
0.000185690609388068	0.38\\
0.000185690609388068	0.39\\
0.000185809971110344	0.39\\
0.000185809971110344	0.4\\
0.000186484144343535	0.4\\
0.000186484144343535	0.41\\
0.000186727973380558	0.41\\
0.000186727973380558	0.42\\
0.000187789617452051	0.42\\
0.000187789617452051	0.43\\
0.000190878716688063	0.43\\
0.000190878716688063	0.44\\
0.000192092391078644	0.44\\
0.000192092391078644	0.45\\
0.0001925708057419	0.45\\
0.0001925708057419	0.46\\
0.000192825329902341	0.46\\
0.000192825329902341	0.47\\
0.00019574668049318	0.47\\
0.00019574668049318	0.48\\
0.000196054427259001	0.48\\
0.000196054427259001	0.49\\
0.000196066120994377	0.49\\
0.000196066120994377	0.5\\
0.000196243712916713	0.5\\
0.000196243712916713	0.51\\
0.000197908542453539	0.51\\
0.000197908542453539	0.52\\
0.000199951866781676	0.52\\
0.000199951866781676	0.53\\
0.000201967012243252	0.53\\
0.000201967012243252	0.54\\
0.000204583495005922	0.54\\
0.000204583495005922	0.55\\
0.000205083620511362	0.55\\
0.000205083620511362	0.56\\
0.000206217822033662	0.56\\
0.000206217822033662	0.57\\
0.000210588176358721	0.57\\
0.000210588176358721	0.58\\
0.000210891628503493	0.58\\
0.000210891628503493	0.59\\
0.000211612889490476	0.59\\
0.000211612889490476	0.6\\
0.000216704452699321	0.6\\
0.000216704452699321	0.61\\
0.00021792486168125	0.61\\
0.00021792486168125	0.62\\
0.00021880506567007	0.62\\
0.00021880506567007	0.63\\
0.000220244805660615	0.63\\
0.000220244805660615	0.64\\
0.000223864472688557	0.64\\
0.000223864472688557	0.65\\
0.000225482117588474	0.65\\
0.000225482117588474	0.66\\
0.000235902796234541	0.66\\
0.000235902796234541	0.67\\
0.000236873568457471	0.67\\
0.000236873568457471	0.68\\
0.000238717174074063	0.68\\
0.000238717174074063	0.69\\
0.000240600914805742	0.69\\
0.000240600914805742	0.7\\
0.000242010799241503	0.7\\
0.000242010799241503	0.71\\
0.000248589256914538	0.71\\
0.000248589256914538	0.72\\
0.000248853053106988	0.72\\
0.000248853053106988	0.73\\
0.000249579117032489	0.73\\
0.000249579117032489	0.74\\
0.00025030545113763	0.74\\
0.00025030545113763	0.75\\
0.000251515601330918	0.75\\
0.000251515601330918	0.76\\
0.000255359436627307	0.76\\
0.000255359436627307	0.77\\
0.000255591279058822	0.77\\
0.000255591279058822	0.78\\
0.000257462691045095	0.78\\
0.000257462691045095	0.79\\
0.000259044884009224	0.79\\
0.000259044884009224	0.8\\
0.000263163762063586	0.8\\
0.000263163762063586	0.81\\
0.000265082226469375	0.81\\
0.000265082226469375	0.82\\
0.000270683907654262	0.82\\
0.000270683907654262	0.83\\
0.000271794779947823	0.83\\
0.000271794779947823	0.84\\
0.000274334055882935	0.84\\
0.000274334055882935	0.85\\
0.000275601789897137	0.85\\
0.000275601789897137	0.86\\
0.00027659085624157	0.86\\
0.00027659085624157	0.87\\
0.000276598188193763	0.87\\
0.000276598188193763	0.88\\
0.000279274580375057	0.88\\
0.000279274580375057	0.89\\
0.000284652041007721	0.89\\
0.000284652041007721	0.9\\
0.000289244724459333	0.9\\
0.000289244724459333	0.91\\
0.000294055228010513	0.91\\
0.000294055228010513	0.92\\
0.000295103004695487	0.92\\
0.000295103004695487	0.93\\
0.000301143470761249	0.93\\
0.000301143470761249	0.94\\
0.000306698642341025	0.94\\
0.000306698642341025	0.95\\
0.000309825544728867	0.95\\
0.000309825544728867	0.96\\
0.000312107851901522	0.96\\
0.000312107851901522	0.97\\
0.000317339375649714	0.97\\
0.000317339375649714	0.98\\
0.000352791213145002	0.98\\
0.000352791213145002	0.99\\
0.295800980029507	0.99\\
0.295800980029507	1\\
inf	1\\
};
\addplot [color=mycolor3, forget plot,line width=1.5]
  table[row sep=crcr]{%
-inf	0\\
0.000169451932988865	0\\
0.000169451932988865	0.01\\
0.000170869657332569	0.01\\
0.000170869657332569	0.02\\
0.000173156469361578	0.02\\
0.000173156469361578	0.03\\
0.000174930582071079	0.03\\
0.000174930582071079	0.04\\
0.000176567069641178	0.04\\
0.000176567069641178	0.05\\
0.000177092734381889	0.05\\
0.000177092734381889	0.06\\
0.000178180324037252	0.06\\
0.000178180324037252	0.07\\
0.000178739405469641	0.07\\
0.000178739405469641	0.08\\
0.000178782934322459	0.08\\
0.000178782934322459	0.09\\
0.000179225418848838	0.09\\
0.000179225418848838	0.1\\
0.00017936980249678	0.1\\
0.00017936980249678	0.11\\
0.000179690545128542	0.11\\
0.000179690545128542	0.12\\
0.000181061753011422	0.12\\
0.000181061753011422	0.13\\
0.000181315210818848	0.13\\
0.000181315210818848	0.14\\
0.000182595537689047	0.14\\
0.000182595537689047	0.15\\
0.000183208590238391	0.15\\
0.000183208590238391	0.16\\
0.000183695248950714	0.16\\
0.000183695248950714	0.17\\
0.000183759674345899	0.17\\
0.000183759674345899	0.18\\
0.000184069244218566	0.18\\
0.000184069244218566	0.19\\
0.000184594198040962	0.19\\
0.000184594198040962	0.2\\
0.000186004387195599	0.2\\
0.000186004387195599	0.21\\
0.000186072700172296	0.21\\
0.000186072700172296	0.22\\
0.000186418358382107	0.22\\
0.000186418358382107	0.23\\
0.000187648663810391	0.23\\
0.000187648663810391	0.24\\
0.000189327266663453	0.24\\
0.000189327266663453	0.25\\
0.00019040945629639	0.25\\
0.00019040945629639	0.26\\
0.000191068345025673	0.26\\
0.000191068345025673	0.27\\
0.000191305308792704	0.27\\
0.000191305308792704	0.28\\
0.000192501150514091	0.28\\
0.000192501150514091	0.29\\
0.000192722218123993	0.29\\
0.000192722218123993	0.3\\
0.000193626695705274	0.3\\
0.000193626695705274	0.31\\
0.000194419278937604	0.31\\
0.000194419278937604	0.32\\
0.000194597724918652	0.32\\
0.000194597724918652	0.33\\
0.000194890336433903	0.33\\
0.000194890336433903	0.34\\
0.000195886119089187	0.34\\
0.000195886119089187	0.35\\
0.000197398180765593	0.35\\
0.000197398180765593	0.36\\
0.000197642912999712	0.36\\
0.000197642912999712	0.37\\
0.000198134754562639	0.37\\
0.000198134754562639	0.38\\
0.000198211078143339	0.38\\
0.000198211078143339	0.39\\
0.000199969031674611	0.39\\
0.000199969031674611	0.4\\
0.000200471637934734	0.4\\
0.000200471637934734	0.41\\
0.000200778820591404	0.41\\
0.000200778820591404	0.42\\
0.000200966776759283	0.42\\
0.000200966776759283	0.43\\
0.000201051526602986	0.43\\
0.000201051526602986	0.44\\
0.000202693726358974	0.44\\
0.000202693726358974	0.45\\
0.000203331707488145	0.45\\
0.000203331707488145	0.46\\
0.000203629403148983	0.46\\
0.000203629403148983	0.47\\
0.000203955028517735	0.47\\
0.000203955028517735	0.48\\
0.000205639339371028	0.48\\
0.000205639339371028	0.49\\
0.000207847061506499	0.49\\
0.000207847061506499	0.5\\
0.00021305485584712	0.5\\
0.00021305485584712	0.51\\
0.000213061313424855	0.51\\
0.000213061313424855	0.52\\
0.000213984108915761	0.52\\
0.000213984108915761	0.53\\
0.000215250908037233	0.53\\
0.000215250908037233	0.54\\
0.000215264494991469	0.54\\
0.000215264494991469	0.55\\
0.00021611685383286	0.55\\
0.00021611685383286	0.56\\
0.000218414461217534	0.56\\
0.000218414461217534	0.57\\
0.000218510731902112	0.57\\
0.000218510731902112	0.58\\
0.000220054823579761	0.58\\
0.000220054823579761	0.59\\
0.000220462096759053	0.59\\
0.000220462096759053	0.6\\
0.00022091241256949	0.6\\
0.00022091241256949	0.61\\
0.000221304140312445	0.61\\
0.000221304140312445	0.62\\
0.000222442056363868	0.62\\
0.000222442056363868	0.63\\
0.000223730765778116	0.63\\
0.000223730765778116	0.64\\
0.000225108971793075	0.64\\
0.000225108971793075	0.65\\
0.00022650347862618	0.65\\
0.00022650347862618	0.66\\
0.000228064338606816	0.66\\
0.000228064338606816	0.67\\
0.000229180995349608	0.67\\
0.000229180995349608	0.68\\
0.00022946257084252	0.68\\
0.00022946257084252	0.69\\
0.000229884808400469	0.69\\
0.000229884808400469	0.7\\
0.000230741162581845	0.7\\
0.000230741162581845	0.71\\
0.000231019748245648	0.71\\
0.000231019748245648	0.72\\
0.000231063652675362	0.72\\
0.000231063652675362	0.73\\
0.000233995913554055	0.73\\
0.000233995913554055	0.74\\
0.000241289868582132	0.74\\
0.000241289868582132	0.75\\
0.000241471595774144	0.75\\
0.000241471595774144	0.76\\
0.000242252936494447	0.76\\
0.000242252936494447	0.77\\
0.000242539790876054	0.77\\
0.000242539790876054	0.78\\
0.000242875602992037	0.78\\
0.000242875602992037	0.79\\
0.000244766266441542	0.79\\
0.000244766266441542	0.8\\
0.000246993918881895	0.8\\
0.000246993918881895	0.81\\
0.000248131826193716	0.81\\
0.000248131826193716	0.82\\
0.000249004126418729	0.82\\
0.000249004126418729	0.83\\
0.000251662570457004	0.83\\
0.000251662570457004	0.84\\
0.000253209340812731	0.84\\
0.000253209340812731	0.85\\
0.000254596684461822	0.85\\
0.000254596684461822	0.86\\
0.000254789408126122	0.86\\
0.000254789408126122	0.87\\
0.000256474968321403	0.87\\
0.000256474968321403	0.88\\
0.000257033885416166	0.88\\
0.000257033885416166	0.89\\
0.000262301382543647	0.89\\
0.000262301382543647	0.9\\
0.000264877487134934	0.9\\
0.000264877487134934	0.91\\
0.000270757241380963	0.91\\
0.000270757241380963	0.92\\
0.000281336069929461	0.92\\
0.000281336069929461	0.93\\
0.000290909833815923	0.93\\
0.000290909833815923	0.94\\
0.000292632780932241	0.94\\
0.000292632780932241	0.95\\
0.000312570101551869	0.95\\
0.000312570101551869	0.96\\
0.000335229906777619	0.96\\
0.000335229906777619	0.97\\
0.000338043068859436	0.97\\
0.000338043068859436	0.98\\
0.000357779962321375	0.98\\
0.000357779962321375	0.99\\
0.00043819838807345	0.99\\
0.00043819838807345	1\\
inf	1\\
};
\end{axis}


==> pebs.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
\definecolor{mycolor1}{rgb}{0.00000,0.44700,0.74100}%
\definecolor{mycolor2}{rgb}{0.85000,0.32500,0.09800}%
\definecolor{mycolor3}{rgb}{0.92900,0.69400,0.12500}%
\definecolor{mycolor4}{rgb}{0.49400,0.18400,0.55600}%
%

\begin{axis}[%
at={(-2.1cm,0cm)},
width=4.5cm,
height=4cm,
scale only axis,
xmode=log,
xmin=1,
xmax=50,
xminorticks=true,
ymode=log,
ymin=1e-05,
ymax=1,
yminorticks=true,
xlabel={\footnotesize a) $d [\mathrm{m}] $},
axis background/.style={fill=white},
axis x line*=bottom,
axis y line*=left,
xmajorgrids,
xminorgrids,
ymajorgrids
]
\node[rotate=40,fill=white] at (axis cs:5,.002) {\footnotesize Random };
\node[rotate=40,fill=white] at (axis cs:5,.0001) {\footnotesize Directional };
\draw (axis cs:5.5,.00004) ellipse (.1cm and .2cm);
\draw (axis cs:5,.0005) ellipse (.1cm and .2cm);
\addplot [color=mycolor1, forget plot,line width=1.5]
  table[row sep=crcr]{%
1	6.63281576565766e-06\\
1.27427498570313	1.24571876487842e-05\\
1.62377673918872	2.36650160410122e-05\\
2.06913808111479	4.62631554608735e-05\\
2.63665089873036	9.21629543630577e-05\\
3.35981828628378	0.000183484676614509\\
4.28133239871939	0.00037425910813291\\
5.45559478116852	0.00077568945676615\\
6.95192796177561	0.00159952316003032\\
8.85866790410082	0.00328525775217572\\
11.2883789168469	0.00682172379372616\\
14.3844988828766	0.013979385767212\\
18.3298071083244	0.0291163506771437\\
23.3572146909012	0.0597000312530902\\
29.7635144163132	0.124474080972064\\
37.9269019073225	0.255889550119898\\
48.3293023857175	0.533321161619385\\
61.5848211066026	1.08915903729389\\
78.4759970351461	2.25149374807732\\
100	4.71593981321998\\
};
\addplot [color=mycolor2, only marks, mark=square, mark options={solid, mycolor2}, forget plot,line width=1.5]
  table[row sep=crcr]{%
1	6.72279038578006e-06\\
1.27427498570313	1.23268703824158e-05\\
1.62377673918872	2.38731891207223e-05\\
2.06913808111479	4.57529020429913e-05\\
2.63665089873036	9.31246022913377e-05\\
3.35981828628378	0.000176224624070884\\
4.28133239871939	0.000376478356951156\\
5.45559478116852	0.000769662324158172\\
6.95192796177561	0.00156175716162269\\
8.85866790410082	0.00318097867570969\\
11.2883789168469	0.0067711843946802\\
14.3844988828766	0.0136858058334389\\
18.3298071083244	0.0293652801743878\\
23.3572146909012	28.7318112776332\\
29.7635144163132	65.9973667580549\\
37.9269019073225	69.542719287805\\
48.3293023857175	72.9168174196587\\
61.5848211066026	76.5911097870799\\
78.4759970351461	88.4599553841714\\
100	103.861753045388\\
};
\addplot [color=mycolor3, forget plot,line width=1.5]
  table[row sep=crcr]{%
1	1.12338936370682e-06\\
1.27427498570313	1.87460475005799e-06\\
1.62377673918872	3.04668160942692e-06\\
2.06913808111479	5.37682295309639e-06\\
2.63665089873036	7.92093407968065e-06\\
3.35981828628378	1.38186206893606e-05\\
4.28133239871939	2.49360077906243e-05\\
5.45559478116852	3.76186644506405e-05\\
6.95192796177561	6.33526113773838e-05\\
8.85866790410082	0.000116867060560047\\
11.2883789168469	0.000219882940076596\\
14.3844988828766	0.000454581110384452\\
18.3298071083244	0.00100513740943559\\
23.3572146909012	0.00229589529818709\\
29.7635144163132	0.00559073226515006\\
37.9269019073225	0.0139645885520947\\
48.3293023857175	0.0360221369647204\\
61.5848211066026	0.092204881974793\\
78.4759970351461	0.235965991138321\\
100	0.625172892276431\\
};
\addplot [color=mycolor4, only marks, mark=x, mark options={solid, mycolor4}, forget plot,line width=1.5]
  table[row sep=crcr]{%
1	1.38221325018614e-06\\
1.27427498570313	1.88643231719039e-06\\
1.62377673918872	2.92255144284642e-06\\
2.06913808111479	5.22366805894463e-06\\
2.63665089873036	7.85622834184143e-06\\
3.35981828628378	1.39019470310631e-05\\
4.28133239871939	2.50691962286822e-05\\
5.45559478116852	3.68332357706635e-05\\
6.95192796177561	6.11612065231306e-05\\
8.85866790410082	0.00011617731638305\\
11.2883789168469	0.00316621090381372\\
14.3844988828766	0.000453233372436663\\
18.3298071083244	0.000985942686187251\\
23.3572146909012	0.00222292747353848\\
29.7635144163132	0.00548669383919826\\
37.9269019073225	0.726807941102239\\
48.3293023857175	19.1536801881545\\
61.5848211066026	37.7014872059233\\
78.4759970351461	60.477604664735\\
100	87.1948210503601\\
};
\end{axis}

